Simultaneous Approximation of Constraint Satisfaction Problems

Given $k$ collections of 2SAT clauses on the same set of variables $V$, can we find one assignment that satisfies a large fraction of clauses from each collection? We consider such simultaneous constraint satisfaction problems, and design the first nontrivial approximation algorithms in this context. Our main result is that for every CSP $F$, for $k < \tilde{O}(\log^{1/4} n)$, there is a polynomial time constant factor Pareto approximation algorithm for $k$ simultaneous Max-$F$-CSP instances. Our methods are quite general, and we also use them to give an improved approximation factor for simultaneous Max-w-SAT (for $k <\tilde{O}(\log^{1/3} n)$). In contrast, for $k = \omega(\log n)$, no nonzero approximation factor for $k$ simultaneous Max-$F$-CSP instances can be achieved in polynomial time (assuming the Exponential Time Hypothesis). These problems are a natural meeting point for the theory of constraint satisfaction problems and multiobjective optimization. We also suggest a number of interesting directions for future research.

==> intro.tex <==
\section{Introduction}
% \Sknote{ We should put in a very prominent message saying that: significantly generalized and strengthened from the version of November 2013. It is very standard for reviewers to just copy their old review, assuming that the paper is the same.}
The theory of approximation algorithms for constraint satisfaction
problems (CSPs) is a very central and well developed part of modern
theoretical computer science.  Its study has involved fundamental
theorems, ideas, and problems such as the PCP theorem, linear and
semidefinite programming, randomized rounding, the Unique Games
Conjecture, and deep connections between them~\cite{AroraS98,
  AroraLMSS98, GW-sdp95, Khot02, Raghavendra08, RaghavendraS09}.

In this paper, we initiate the study of {\em simultaneous
  approximation algorithms} for constraint satisfaction problems. A
typical such problem is the simultaneous \maxcut problem: Given a
collection of $k$ graphs $G_i = (V, E_i)$ on the same vertex set $V$, the
problem is to find a single cut (i.e., a partition of $V$) so that in
{\em every} $G_i$, a large fraction of the edges go across the cut.

More generally, let $q$ be a constant positive integer, and let
$\calF$ be a set of bounded-arity predicates on $[q]$-valued
variables. Let $V$ be a set of $n$ $[q]$-valued variables.  An
$\calF$-CSP is a weighted collection $\calW$ of constraints on $V$,
where each constraint is an application of a predicate from $\calF$ to
some variables from $V$.  For an assignment $f: V \to [q]$ and a
$\calF$-CSP instance $\calW$, we let $\val(f, \calW)$ denote the total
weight of the constraints from $\calW$ satisfied by $f$.
%\Ssnote{Change $[q]$ to  $[q]$ everywhere?}

We now describe the setting for the problem we consider:
\emph{$k$-fold simultaneous} {\sc Max}-$\calF$-CSP. Let $\calW_1,
\ldots, \calW_k$ be $\calF$-CSPs on $V$, each with total weight $1$.
Our high level goal is to find an assignment $f: V \to [q]$ for which
$\val(f, \calW_\ell)$ is large for all $\ell \in [k]$.
% \Ssnote{We don't need
%   total weight 1. Or say, wlog, each instance has total weight 1. Or
%   we can stress in the notation section, that the total weight need
%   not be 1.}

These problems fall naturally into the domain of multi-objective
optimization: there is a common search space, and multiple objective
functions on that space.  Since even optimizing one of these objective
functions could be NP-hard, it is natural to resort to approximation
algorithms. Below, we formulate some of the approximation criteria
that we will consider, in decreasing order of difficulty:
%
\begin{enumerate}
\item {\bf Pareto approximation:} 
Suppose $(c_1, \ldots, c_k) \in [0,1]^k$ is such that
there is an assignment $f^*$ with $\val(f^*, \calW_\ell) \geq c_\ell$
for each $\ell \in [k]$.

An $\alpha$-Pareto approximation algorithm in this context is an algorithm,
which when given $(c_1, \ldots, c_k)$ as input, finds an assignment $f$ such that
$\val(f, \calW_\ell) \geq \alpha \cdot c_\ell$, for each $\ell \in [k]$.


\item {\bf Minimum approximation:} This is basically the Pareto
  approximation problem when $c_1 = c_2= \ldots = c_k$. Define $\opt$
  to be the maximum, over all assignments $f^*$, of $\min_{\ell \in
    [k]} \val(f^*, \calW_\ell)$.

  An $\alpha$-minimum approximation algorithm in this context is an
  algorithm which finds an assignment $f$ such that $\min_{\ell \in
    [k]} \val(f, \calW_\ell) \geq \alpha \cdot \opt$.

\item {\bf Detecting Positivity:} This is a very special case of the above,
where the goal is simply to determine whether there is an assignment $f$ which
makes $\val(f, \calW_\ell) > 0$ for all $\ell \in [k]$.

At the surface, this problem appears to be a significant
weakening of the the simultaneous approximation goal.
\end{enumerate}


When $k = 1$, minimum approximation and Pareto approximation correspond
to the classical \maxcsp approximation problems
(which have received much attention). Our focus in this paper is on
general $k$. As we will see in the discussions below, the nature of
the problem changes quite a bit for $k > 1.$  In
particular, direct applications of classical techniques like random
assignments and convex programming relaxations fail to give even a
constant factor approximation.

We have two main motivations for studying simultaneous approximations
for CSPs. Most importantly, these are very natural algorithmic
questions, and capture naturally arising constraints in a way which
more na\"{i}ve formulations (such as taking linear combinations of the
given CSPs) cannot.  Secondly, the study of simultaneous approximation
algorithms for CSPs sheds new light on various aspects of standard
approximation algorithms for CSPs. For example, our algorithms are
able to favorably exploit some features of the trivial
random-assignment-based $\nfrac{1}{2}$-approximation algorithm for
\maxcut, that are absent in the more sophisticated SDP-based
0.878-approximation algorithm of Goemans-Williamson~\cite{GW-sdp95}.

%\Ssnote{The last line above, ``more useful'' seems quite
%  provocative. We should probably tone it down a bit, and specify more
  %clearly what do we mean}


\subsection{Some observations about simultaneous approximation }
We begin with some simple observations about simultaneous CSPs, and
then discuss why a direct application of the classical CSP algorithms 
fails in this setting.
 % \Ssnote{I am not sure if presenting such an
 %  enumerated list of disconnected facts is a good way.}
%
\begin{enumerate}

\item Detecting positivity for $k$-fold simultaneous
\maxfcsp has a trivial $n^{O(k)}$ time algorithm: For every possible
way of choosing one constraint per instance, check if it is possible to satisfy
those constraints.


\item Finding an $\alpha$-Pareto approximation or an $\alpha$-minimum
  approximation to the $k$-fold \maxfcsp is at least as hard as
  finding an $\alpha$-approximation the classical \maxfcsp problem
  (i.e., $k = 1$).  Thus the known limits on polynomial-time
  approximability extend naturally to our setting. \Ssnote{Changed
    this line.}
% Thus there are some known basic limits on the
%   approximation factors achievable in polynomial time.


\item The simplest simultaneous CSP is {\sc Max-1-SAT}. It is easy to
  see that detecting positivity of a $k$-fold simultaneous {\sc
    Max-1-SAT} is exactly the same problem as detecting satisfiability
  of a SAT formula with $k$ clauses. This problem has been studied in
  the fixed parameter tractability literature~\cite{Marx13}, and
  a $2^{O(k)} \cdot \poly(n)$ time algorithm is known for this
  problem. 
% \Ssnote{What is the reference? Are we referring to slides?
%     Is it known that this is tight? It might be worth mentioning if
%     there is a lower bound here.}
% \Sknote{ It is tight .. but that will take away
% the punch from the lower bound. I wasn't able to find a paper with this result
% and the slides don't cite so let us just cite the slides .. it is no big deal.}
% \Sknote{Slides here: http://www.cs.bme.hu/~dmarx/papers/marx-bergen-2013-csp.pdf}

\item The problem of getting a $1$-Pareto or $1$-minimum approximation
  to $k$-fold simultaneous {\sc Max-1-SAT} is essentially the NP-hard
  SUBSET-SUM problem. There is a simple $2^{\poly(k/\epsilon)}\cdot
  \poly(n)$-time $(1-\epsilon)$-Pareto approximation algorithm based
  on dynamic programming. \Ssnote{Are you sure of the reduction to Subsetsum?}
\Sknote{Yeah I think so.}


\item Let us now consider simultaneous approximation algorithms for
  \maxcut.

  First recall the simple random partition algorithm in the classical
  case.  A uniformly random cut in a weighted graph graph cuts
  $\nfrac{1}{2}$ the total weight in expectation. This gives a
  $\nfrac{1}{2}$-approximation to the classical \maxcut problem.

  For an {\em unweighted} graph\footnote{We use the term ``unweighted"
    to refer to instances where all the constraints have the same
    weight.  When we talk about simultaneous approximation for
    unweighted instances $\calW_1, \ldots, \calW_k$ of
    MAX-$\calF$-CSP, we mean that in each instance $\calW_i$, all
    constraints with nonzero weight have the equal weights (but that
    equal weight can be different for different $i$).}  $G$ with
  $\omega(1)$ edges, a simple variance calculation shows that a
  uniformly random cut in the graph cuts a $\left(\frac{1}{2}
    -o(1)\right)$ fraction of the total number of edges {\em with high
    probability}.  Thus, for $k = O(1)$ simultaneous unweighted
  instances $G_1, \ldots, G_k$ of \maxcut, a uniformly random cut
  gives a $\left(\frac{1}{2} - o(1)\right)$-minimum (and Pareto)
  approximation with high probability.

  For {\em weighted} graphs, this algorithm breaks down completely
  (because the concentration no longer holds), and fails to give any
  constant factor approximation.
%\Ssnote{We should explain in a line or two why it breaks down, and
%  that's there's no trivial fix.}

\item The celebrated Goemans-Williamson Semi-Definite Programming
  (SDP) algorithm~\cite{GW-sdp95} gives a $0.878$-approximation to the
  classical \maxcut problem. How does that generalize to the
  simultaneous setting?

There is a natural SDP relaxation that one can write for
simultaneous \maxcut of $G_1,
\ldots, G_k$. Perhaps we can do hyperplane rounding of the vector
solution for this SDP to give us a simultaneously good cut for all the
$G_i$? We know that each $G_i$ will get a good cut in expectation, but
we need each $G_i$ to get a good cut {\em with high probability} to
guarantee a simultaneously good cut.

However, there are cases where the SDP rounding fails completely.  For
weighted instances, the SDP does not have {\em any} constant
integrality gap.
For unweighted instances, for every fixed $k$, we find an instance
of $k$-fold simultaneous \maxcut  (with arbitrarily many vertices and 
edges) where the SDP relaxation has value
$1- \Omega\left(\frac{1}{k^2}\right)$, while the optimal simultaneous
cut has value only $\nfrac{1}{2}$. 
%\Ssnote{maybe ``we construct $k$
%%unweighted  instances of simultaneous max-cut'' and ``arbitrarily many
%edges'' rather than 'vertices'}
Furthermore, applying the hyperplane
rounding algorithm to this vector solution gives (with probability 1)
a simultaneous cut value of {\em 0}. These integrality gaps are
described in Section~\ref{section:sdp}.

Thus the natural extension of SDP based techniques for
simultaneous approximation fail quite spectacularly. A-priori, this
failure is quite surprising, since SDPs (and LPs) generalize to the
multiobjective setting seamlessly. 
% \Ssnote{This line seems too similar
% to the opening line of the second para in this point.}


%Note that our algorithm
%in Theorem~\ref{ adsf }, achieves essentially the same approximation ratio
%as this integrality gap.

\item For general CSPs, the total weight satisfied by a random
  assignment does not necessarily concentrate strongly, even for
  general unweighted instances.  In particular, there is no ``trivial"
  random-assignment-based constant factor approximation algorithm for
  simultaneous general CSPs.
  \Ssnote{I am not sure
    I believe this. For unweighted instance, consider a large
    ``constant degree'' and ``uniform'' instance. The variance would
    be of the order of $1/n.$ }
\Sknote{I made it a little milder. The point was that
for GENERAL instances there is no trivial algorithm .. so if you cheat and make it constant degree uniform then the claim isn't true.} 
\end{enumerate}






\subsection{Results}

%\Ssnote{In this section, we need to make sure it's clear why the
%  theorem is non-trivial. It should be clear that the basic techniques
%fail. For \maxcut, we want to make it clear that the random assignment
%algorithm fails because the cut value may not be concentrated, because
%of a skewed weight distribution. For \maxsat, we need to clarify why
%more ideas are required, and why we need to not just pick heavy
%variables, but also recurse over all possible assignments to the
%picked variables.}

Our results address the approximability of $k$-fold simultaneous
\maxfcsp for large $k$.  Our main algorithmic result shows that for $k
= \log^{O(1)}n$, $k$-fold simultaneous \maxfcsp has a constant
factor Pareto approximation algorithm.
\begin{theorem}
\label{theorem:results:maxcsp}
Let $q, w$ be constants, and let
$\calF$ be a finite set of predicates on $[q]$-valued variables
of arity at most $w$.

Then for every $\epsilon > 0$, 
there is a $2^{O(\nfrac{k^3}{\eps^2}\log(\nfrac{k}{\eps}))} \cdot \poly(n)$-time $\left(\frac{1}{q^{w-1}} - \epsilon \right)$-Pareto
approximation algorithm for $k$-fold simultaneous
\maxfcsp. 
\end{theorem}
%\Ssnote{$w$ is also constant. Use [q] instead of $\Sigma$?}
%\Ssnote{Is this the only theorem we want to state here about the
%  algorithms? This doesn't imply the 2SAT algorithm.}

The proof of this Theorem appears in Section~\ref{section:maxcsp}, and
involves a number of ideas. In order to make the ideas clearer, we
work our way up to the full proof by gradually introducing these ideas
in proofs of simpler results. In Section~\ref{section:max-cut}, using
the simplest versions of our ideas, we give a $(\nfrac{1}{2} -
\epsilon)$-Pareto approximation algorithm for simultaneous \maxcut.
In Section~\ref{section:maxsat}, we combine this basic approach with
linear-programming relaxations to get a $(\nfrac{3}{4} -
\epsilon)$-Pareto approximation algorithm for simultaneous \maxsat.
In Section~\ref{section:maxand}, we introduce some significant
additions to the both the algorithm and the analysis framework to get
a $(\nfrac{1}{2} -\epsilon)$-Pareto approximation for simultaneous
\maxand (this implies the same factor Pareto approximation algorithm
for the general simultaneous {\sc Max-2-CSP}, where every arity-2
predicate on Boolean variables is allowed). Finally, in
Section~\ref{section:maxcsp}, we give the full proof of
Theorem~\ref{theorem:results:maxcsp}.


In contrast to the above approximation algorithms for $k = \log^{O(1)}n$,
we show that when $k = \omega(\log n)$, it is hard to
obtain any constant factor approximation whatsoever to the $k$-fold
simultaneous {\sc Max}-$w$-CSP problem in polynomial time.

More precisely, we show that for every ``nontrivial" collection of
Boolean predicates $\calF$, even detecting positivity for simultaneous
\maxfcsp instances is hard. This enables us implies a complete {\em
  dichotomy theorem} for constant factor approximations of $k$-fold
simultaneous Boolean CSPs, for $k = \log^{\Omega(1)} n$.
 


%Let
%$\calF$ be a finite set of predicates. An instance of the $k$-fold
%simultaneous MAX-$\calF$-CSP problem is given by $k$ collections
%$\calC_1, \ldots, \calC_k$, of constraints on the variables $x_1,
%\ldots, x_n$, where each constraint is an application of a predicate
%from $\calF$ on some subset of the variables


A predicate $P: \{0,1\}^w \to \{\true, \false\}$ is said to be {\em
  $0$-valid}/{\em $1$-valid} if the
all-$0$-assignment/all-$1$-assignment satisfies $P$. We call a
collection $\calF$ of predicates {\em $0$-valid}/{\em $1$-valid} if
all predicates in $\calF$ are $0$-valid/$1$-valid.  Clearly, if
$\calF$ is $0$-valid or $1$-valid, the simultaneous \maxfcsp instances
can be solved exactly (by considering the
all-$0$-assignment/all-$1$-assignment). Our next theorem shows that
detecting positivity of $\omega(\log n)$-fold simultaneous \maxfcsp,
for all other $\calF$, is hard.
%
\begin{theorem}
\label{thm:dichotomy}
Assume the Exponential Time Hypothesis~\cite{ImpagliazzoP01, ImpagliazzoPZ01}. Let $\calF$ be a fixed finite
set of Boolean predicates. If $\calF$ is not $0$-valid or $1$-valid,
then for $k = \omega(\log n )$, detecting positivity of $k$-fold
simultaneous \maxfcsp on $n$ variables requires time superpolynomial
in $n$.
\end{theorem}
%\Ssnote{We should state the ETH somewhere, maybe in the hardness section.}

Crucially, this hardness result holds even if we require
that every predicate in an instance has all its inputs being {\em distinct variables}.
%\footnote{Without this requirement,
%for many $\calF$ the hardness basically follows from the hardness of simultaneous MAX-1-SAT;
%this hardness reduction does not seem to capture the true nature of max-$\calF$-CSP.}.



% \Ssnote{There is actually a small issue to note here. There are $k$
%   instances on $\Theta(k)$ variables and with only a constant number
%   of constraints in each of the instances, already requires time
%   superpolynomial in $n$ for $k = \omega(\log n).$ Currently we are
%   interpreting this as $\omega(\log n)$ instances on $n$
%   variables. One things that's not coming out in the current
%   statements is that the instance sizes are not unreasonably large
%   (right now they could in fact be superpolynomial in $n$). }


Our proof uses techniques underlying the dichotomy
theorems of Schaefer~\cite{Schaefer78} for exact CSPs, and of Khanna
\etal~\cite{KhannaSTW01} for {\sc Max}-CSPs (although our easiness criterion
is different from the easiness criteria in both these papers).



\paragraph{Remarks}
\begin{enumerate}

\item In particular, our result implies a $2^{\poly(k)}\cdot \poly(n)$
  time algorithm for detecting positivity of $k$-fold simultaneous
  \maxfcsp (improving on the trivial $n^{O(k)}$ time algorithm).  For
  this special case, our algorithm and analysis could be simplified
  somewhat (but not much).

\item This improved algorithm for detecting positivity has applications to checking satisfiability of
certain depth-3 Boolean formulas.


\noindent{\bf Theorem: } Given a Boolean circuit of depth 3, where the
top gate is an AND gate with fan-in $k$, the next level consists of OR
gates, and the bottom level consists of AND gates with $O(1)$ fan-in,
one can determine in $2^{\poly(k)} \cdot \poly(n)$ time whether this
circuit is satisfiable. 

As mentioned earlier, detecting positivity for simultaneous {\sc
  Max-1-SAT} turns out to be equivalent to solving SAT on $k$ clauses
(and it was known that this is fixed-parameter tractable, i.e., it can be solved in time $2^{O(k)}\cdot \poly(n)$).
This FPT result has motivated several generalizations and
directions~\cite{sat-fpt1, sat-fpt2, sat-fpt3}. Our satisfiability
algorithm above gives a different generalization which seems
interesting in its own right. 

\item If one only wanted a $n^{\poly(k/\epsilon)}$ running time in
  Theorem~\ref{theorem:results:maxcsp}, then this could simplify our
  algorithm and analysis somewhat (but not much).

\item One could also consider the problem of achieving simultaneous
  approximations with an $\alpha$-multiplicative and
  $\epsilon$-additive error. This problem can be solved
by a significantly simpler algorithm and analysis (but note that
this variation does not even yield an algorithm for detecting positivity).
% \Ssnote{I think additive
%  approximations are considerably simpler. You don't need to do any
%  perturbation etc, just remove heavy vertices until the remaining
%  weight is tiny.}
\end{enumerate}

\subsubsection{Simultaneous approximations via SDPs}

It is a tantalizing possibility that one could use SDPs to improve the
LP-based approximation algorithms that we develop.  Especially for constant
$k$, it is not unreasonable to expect that one could obtain a constant
factor Pareto or minimum approximation, for $k$-fold simultaneous
CSPs, better than what can be achieved by linear programming methods.


In this direction, we show how to use simultaneous SDP relaxations
to obtain a polynomial time $(\frac{1}{2} + \Omega(1/k^2))$-minimum approximation
for $k$-fold simultaneous \maxcut on {\em unweighted graphs}.
\begin{theorem}
\label{theorem:results:unweightedmc}
For large enough $n$, there is an algorithm that, given $k$-fold simultaneous unweighted
\maxcut instances on $n$ vertices, runs in time $2^{2^{2^{O(k)}}}
\cdot \poly(n),$ and computes a $\left(\frac{1}{2} +
  \Omega\left(\frac{1}{k^2}\right)\right)$-minimum approximation.
\end{theorem}








\subsection{Our techniques}


We now give an overview of some of the ideas that go into our algorithms and
their analysis. 



We begin with our simplest algorithm, which is for simultaneous
\maxcut.  Let $V$ be the set of variables. We have $k$ instances of
\maxcut.  Consider a uniformly random assignment to the variables.  We
know that for each of the given instances, this random assignment
satisfies $\frac{1}{2}$ the cut constraints in expectation. If we know
(for some reason) that for each instance, about $\nfrac{1}{2}$ the cut
constraints are satisfied {\em with high probability}, then we would
be able to conclude, by a union bound, that a random assignment
simultaneously satisfies about $\nfrac{1}{2}$ the constraints in each
of the instances simultaneously.

So we estimate, for each instance, the variance of the total weight of
satisfied constraints satisfied by the random assignment. If this
variance is small for each instance, we get the desired concentration,
and the above argument works.  Unravelling the variance estimation, it
turns out that the only way the variance can be large is if there is
some variable $v$, such that the total weight of all constraints
containing $v$ is a constant fraction of the total weight of all
constraints. This variable is clearly very important; we thus take it
out and put it into a set $S$.  This process is repeated; we estimate
the expectation and variance of the uniformly random assignment to the
variables of $V \setminus S$ (assuming an arbitrary assignment to the
variables of $S$). If all instances turn out to have their satisfied
weight strongly concentrated, we are happy. Otherwise, we find a
variable which is important for some instance, and move it into $S$.
We stop this process when all the instances either have the
concentration property, or have had many of their important variables
brought into $S$.

The algorithm concludes by taking a uniformly random assignment to the
variables of $V\setminus S$, and trying out all possible assignments
to the variables of $S$.  By construction of $S$, for each instance
either the cut value of the uniformly random assignment will be
strongly concentrated, or else we know that many important variables
of that instance have been brought into $S$.  For the analysis, we
would like to say that if $f^\star : V \to \{0,1\}$ is the ``optimal
assignment", then the algorithm will find a good Pareto approximation
when it tries out the assignment $f^\star |_S$ to the variables of
$S$. For the strongly concentrated instances this is true,
but not for the remaining instances. Instead, we use the ``many important vertices in $S$"
property of the non-concentrated instances to argue that there is a small {\em
  perturbation} $h: S \to \{0,1\}$ of $f^\star|_S$, such that when the
algorithm tries assigning $h$ to the variables of $S$, it finds a good
Pareto approximation.

Next, in Section~\ref{section:maxsat}, we give our $(\nfrac{3}{4} -
\epsilon)$-Pareto approximation algorithm for simultaneous \maxsat.
The key new ingredient in this algorithm (over the algorithm for
simultaneous \maxcut) is the use of a simultaneous LP relaxation. Here
we use the Goemans-Williamson LP relaxation for
\maxsat~\cite{GW-maxsat}, combined with a algorithm of
Trevisan~\cite{Trevisan98} for rounding fractional solutions to this
LP (which has the property that each variable is rounded independently
and from a not-too-biased distribution). The main change from the
algorithm for simultaneous \maxcut is that instead of assigning the
variables in $V \setminus S$ uniformly at random, these variables get
assigned according to the rounding algorithm applied to a solution to
the LP.

%\Ssnote{Should we instead start with pointing out why that this approach
%  fails with MAXAND, rather than just state it? }
In Section~\ref{section:maxand}, we give our algorithm for
$(\nfrac{1}{2} - \epsilon)$-Pareto approximation \maxand (which
implies a $(\nfrac{1}{2}-\epsilon)$-Pareto approximation for general
simultaneous {\sc Max-2-CSP}).  The nature of simultaneous \maxand is
significantly different from \maxcut and \maxsat.  For example, it is
possible to have several instances of \maxand, where each instance has
an unbounded number of constraints, but for which there is no
assignment that satisfies at least one constraint in each instance.

This forces us to introduce several new ideas in both the algorithm
and the analysis.  For one, we need to not only maintain a set $S$ of
important variables, but we also need to maintain an assignment to the
variables of $S$. In the algorithm, this is implemented by maintaining
a tree of possible evolutions; whenever we bring a variable into $S$
(because for some instance the satisfied weight under a random
assignment to $V\setminus S$ is not concentrated), we consider
assigning it both $0$ and $1$, and proceed with both
possibilities. Once the process for creating $S$ and the assignment to
it has finished, we use an LP due to Trevisan for \maxand (which also
comes with a ``good" rounding algorithm for our purposes) to assign
values to the variables in $V \setminus S$.

The analysis proceeds according to the same high-level plan, but with
several subtleties.  For the instances that are well concentrated, we
know that the LP-rounded assignment to $V \setminus S$ will
simultaneously satisfy a large fraction of the weight. For the other
instances, we need to perform a perturbation to the optimal
$f^\star|_S$ so as to ensure that these instances have a lot of weight
satisfied. This perturbation uses the fact that non-concentrated
instances have many important variables in $S$.  Here we have to deal
with two kinds of important variables $x \in S$: those that have a lot
of weight on constraints involving $x$ and another variable from $S$
(this is the only kind of important variable in the \maxcut and
\maxsat cases), and those that have a lot of weight on constraints
involving $x$ and variables from $V\setminus S$. We argue that the
former important variables can be perturbed in a manner similar to
what we do for \maxcut and \maxsat. For the latter important variables however, we
use (for the second time!) the randomness of the assignment to $V
\setminus S$, to argue that they can be perturbed favorably.


Finally, in Section~\ref{section:maxcsp}, we give our full approximation
algorithm for general simultaneous {\sc Max}-$\calF$-CSP.  With the right
abstractions and tools, the algorithm is a natural generalization of
the algorithm for simultaneous \maxand.





\subsection{Related Work}

The theory of {\em exact} multiobjective optimization has been very well studied, 
(see eg.~\cite{PapadimitriouY00, Diakonikolas11} and the references
therein). 

The only prior work on simultaneous approximation algorithms for CSPs
was for the problem of simultaneous \maxcut.  For two graphs, Angel
et. al.~\cite{Angel06} gave a $0.439$-Pareto approximation algorithm.
Bollob\'{a}s and Scott~\cite{BollobasS04} asked what is the largest
simultaneous cut in two unweighted graphs with $m$ edges each. Kuhn
and Osthus~\cite{KuhnO07}, using the second moment method, proved that
for $k$ simultaneous unweighted instances, there is a simultaneous cut
that cuts at least $m/2 - O(\sqrt{km})$ edges in each instance, and
give a deterministic algorithm to find it (this leads to a
$(\frac{1}{2} - o(1))$-Pareto approximation for unweighted instances
with sufficiently many edges).  Our main theorem implies the same
Pareto approximation factor for simultaneous \maxcut on general
weighted instances, while for $k$-fold simultaneous \maxcut on
unweighted instances, our Theorem~\ref{theorem:results:unweightedmc} gives a
$\left(\frac{1}{2} + \Omega(\frac{1}{k^2})\right)$-minimum
approximation algorithm.







% Note that since our algorithm outputs a cut of value
% $\left(\nfrac{1}{2}-\eps\right)$ times the total weight of each instance,
%   our algorithm gives a better guarantee. 
% Their definition of a
%   randomized approximation algorithm is incomparable to our setting.


%A few graph theory papers  have studied the existence of
%simultaneous large cuts in unweighted graphs. Bollob\'{a}s and
%Scott~\cite{BollobasS04} asked what is the largest simultaneous cut in
%two unweighted graphs with $m$ edges each. Kuhn and
%Osthus~\cite{KuhnO07}, using the second moment method, proved that for
%$k$ simultaneous unweighted instances, there is a simultaneous cut
%that cuts at least $m/2 - O(\sqrt{km})$ edges in each instance, and
%give a deterministic algorithm to find it. This implies a factor
%$\left(\frac{1}{2} - \epsilon\right)$ approximation for unweighted
%MAXCUT instances where each graph has sufficiently many edges.







\iffalse{
\subsection{Old}


The main idea behind our algorithms is simultaneous regularization of
the instances. The motivation for this algorithm is the simple
random assignment algorithm: if each instance
happened to be such that the objective value of a random assignment 
was highly concentrated around its mean, then a random assignment
would simultaneously have good objective value in all the instances.

At the high level, we want to partition the search
space $\{0,1\}^V$ into a small number of regions,
such that each region has this good concentration property for each instance.
More concretely, we try to find a set $S \subseteq V$ of constant size,
such that for {\em every} partial assignment to $S$, the objective value of
a random assignment to the variables of $V\setminus S$ is highly concentrated.

Unfortunately, such an attempt is too optimistic. Instead we get a weaker
property, which roughly gives that each instance is either (1) low-variance (i.e., the random assignment's objective value strongly concentrates), or (2) 
high-variance but whose total weight inside $V\setminus S$ is controlled.
It is important for our running time that such a set $S$ can be found
in $n^c$ time for fixed $c$.
Our algorithm then tries all possible partial assignments to $S$, and then
tries to complete this to a full assignment to all of $V$.
In the case of \maxcut, we then take a uniformly random assignment for the
variables outside $S$. In the case of MAX2SAT, we write a linear programming
relaxation for finding the best possible assignment to the variables outside $S$
(given the tried assignment to the variables in $S$), and then perform randomized rounding of the LP solution.

The analysis proceeds by starting with the optimal assignment $f^*$
restricted to $S$. For low-variance instances, we know that the variance
of the random assignment/randomized-rounding is low, and thus 
we get a simultaneously good approximation with high probability. For high-variance
instances, we exploit our control on the amount of their weight in $V\setminus S$. The analysis {\em perturbs} $f^*$ in a certain way
so that it does not affect the low-variance
instances, but satisfies a nontrivial fraction of weight in each of the high-variance instances. The existence of this perturbation crucially uses the way in which $S$ was chosen.

}\fi






%%% This are comments that I (Sushant) need for working with emacs
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "new-simopt"
%%% End: 



==> max2sat.tex <==
\section{Simultaneous \maxsat}
\label{section:maxsat}
In this section, we give our algorithm for simultaneous \maxsat.
{\color{red}The algorithm follows the basic paradigm from \maxcut, but
uses an LP to boost the Pareto approximation factor from
$\left( \frac{1}{2} - \epsilon \right)$ to $\left(\frac{3}{4} - \epsilon \right)$.
}
\subsection{Preliminaries}

%Section~\ref{sec:notation-1}, we define some additional notation for
%this section.

Let $V$ be a set of $n$ Boolean variables. Define $\calC$ to be the
set of all possible 2-SAT constraints on the $n$ variable set $V$.
A \maxsat instance is then described by a weight
function $\calW : \calC \to \rea_{\geq 0}$ (here $\calW(C)$ denotes
the weight of the constraint $C$). We will assume that $\sum_{C \in
  \calC} \calW(C) = 1$.

We say $v \in C$ if the variable $v$ appears in the constraint
$C$. For a constraint $C$, let $C^+$ (resp.  $C^-$) denote the set of
variables $v \in V$ that appear unnegated (resp. negated) in the
constraint $C$.

%\paragraph{Constraints and $\val$}
Let $f: V \to \{0,1\}$ be an assignment. For a constraint $C \in
\calC,$ define $C(f)$ to be 1 if the constraint $C$ is satisfied by
the assignment $f$, and define $C(f) = 0$ otherwise. Then, we have the
following expression for $\val(f,\calW)$:
$$\val(f,\calW) \defeq \sum_{C \in \calC} \calW(C) \cdot C(f).$$

\subsubsection{Active Constraints}
Our algorithm will maintain a small set $S \subseteq V$ of variables,
for which we will try all assignments by brute-force, and then use a
randomized rounding procedure for a linear program to obtain an
assignment for $V \setminus S$. We now introduce some notation for
dealing with this.

Let $S \subseteq V$. We say a constraint $C \in \calC$ is active given
$S$ if at least one of the variables of $C$ is in $V\setminus S$.  We
denote by $\Act(S)$ the set of constraints from $\calC$ which are
active given $S$.  For two constraints $C_1,C_2 \in \calC,$ we say
$C_1 \sim_{S} C_2$ if they share a variable that is contained in $V
\setminus S$. Note that if $C_1 \sim_{S} C_2,$ then $C_1, C_2$ are
both in $\Act(S)$. For two partial assignments $f_1 : S \to \B$ and
$f_2 : V\setminus S \to \B$, let $f = f_1\cup f_2$ is an assignment
$f : V \to \B$ such that $f(x) = f_1(x)$ if $x\in S$ otherwise
$f(x) = f_2(x)$.

Define the active degree of a variable $v \in V\setminus S$ given $S$ by:
$$\activedeg_S(v, \calW) \defeq \sum_{ C \in \Act(S), C \owns v} \calW(C).$$
We then define the active degree of the whole instance $\calW$ given $S$:
$$\activedeg_S(\calW) \defeq \sum_{v \in V\setminus S} \activedeg_{S}(v,
\calW).$$
For a partial assignment $h: S \to \{0,1\}$, we define
$$\val(h,\calW) \defeq  \sum_{\substack{C \in \calC \\  C \notin \Act(S)}} \calW(C) \cdot C(h).$$
Thus, for an assignment $g: V\setminus S \to \{0,1\}$, to the
remaining set of variables, we have the equality:
$$\val(h\cup g,\calW) - \val(h,\calW) = \sum_{C \in \Act(S)}\calW(C) \cdot C(h\cup g).$$

\subsubsection{LP Rounding}
Let $h: S \to \{0,1\}$ be a partial assignment.  We will use the
Linear Program $\LLsat_1(h)$ to complete the assignment to $V
\setminus S$.  Goemans and Williamson~\cite{GW-maxsat} showed, via a
rounding procedure, that this LP can be used to give a $\nfrac{3}{4}$
approximation to MAX2SAT. We will be using a different rounding
procedure, due to Trevisan~\cite{Trevisan98}, that also gives a
$\nfrac{3}{4}$ approximation but has the advantage of being smooth in
a certain sense.

Let $\vec{t}, \vec{z}$ be a feasible solution to the LP
$\LLsat_1(h)$. Let $\smooth(\vec{t})$ denote the map $p: V \setminus
S \to [0,1]$ given by: $p(v) = \frac{1}{4} + \frac{t_v}{2}$.  Note
that $p(v) \in [\nfrac{1}{4}, \nfrac{3}{4}]$ for all $v$.
%For a fractional assignment $p: V\setminus S \to [0,1]$,
%define $\val(p,\calW)$ by:
%\[\val(p,\calW) \defeq \sum_{C \in \calC} \calW(C) \cdot z(C),\]
%%\[\mbox { where } \quad 
%z(C) \defeq \min\{ 1, \sum_{v \in C^+} p(v) + \sum_{v \in C^-}
%(1-p(v)) \}.\] Note that if $p$ is $\{0,1\}$ valued assignment, then
%the above definition is consistent with the original definition of
%$\val(p,\calW)$.
%
\begin{theorem}
\label{thm:sattrev}
Let $h: S \to \{0,1\}$ be a partial assignment.
\begin{enumerate}
\item For every $g_0 : V \setminus S \to \{0,1\}$, there exist
$\vect$, $\vecz$ satisfying $\LLsat_1(h)$ such that for every
\maxsat instance $\calW$:
$$ \sum_{C \in \calC} \calW(C) z_C = \val(g_0 \cup h, \calW).$$
\item Suppose $\vect, \vecz$ satisfy $\LLsat_1(h)$. Let $p =
  \smooth(\vec{t})$.  Then for every \maxsat instance $\calW$:
  \[ \av_g[\val(h \cup g, \calW) ] \geq \frac{3}{4} \cdot \sum_{C \in
    \calC} \calW(C)z_C,\] where $g: V\setminus S \to \{0,1\}$ is such
  that each $g(v)$ is sampled independently with $\E[g(v)] = p(v)$.
  % \Sknote{ Should understand the difference between $\E[\val(h \cup
  %   g)] - \val(h)$ and $\E[\val(h \cup g)]$. Which one do we prove,
  %   which one do we need?}
\end{enumerate}
\end{theorem}
% We omit the proof, because a very similar statement is proved in 
% the next section. 
\Ssnote{Edit this line.}
A very similar statement is proved in the next section, and so we omit
the proof.

\subsection{Random Assignments}
\label{section:maxsat:random}
We now give a sufficient condition
%(very similar to the \maxcut case)
for the value of a \maxsat instance to be highly concentrated under a
{\em sufficiently smooth} independent random assignment to the
variables of $V \setminus S$ (This smooth distribution will come from
the rounding algorithm for the LP). When the condition does not hold,
we will get a variable of high active degree.



Let $S \subseteq V$, and let $h: S \to \{0,1\}$ be an arbitrary
partial assignment to $S$.  Let $p: V \setminus S \to [0,1]$ be such
that $p(v) \in [\nfrac{1}{4}, \nfrac{3}{4}]$ for each $v \in V
\setminus S$. Consider the random assignment $g: V \setminus S \to
\{0,1\}$, where for each $v \in V\setminus S$, $g(v) \in \{0, 1\}$ is
sampled independently with $\E[g(v)] = p(v)$. Define the random
variable
$$Y \defeq \val(h\cup g,\calW) - \val(h,\calW) = \sum_{C \in \Act(S)} \calW(C)\cdot C(h\cup g).$$
The random variable $Y$ measures the contribution of active
constraints to the instance $\calW$.

% As in the last section, we define the random variable
% $$Y \defeq \val(h\cup g,\calW) - \val(h,\calW) = \sum_{C \in \Act(S)} \calW(C)\cdot C(h\cup g),$$
% to measure the contribution of active constraints to the instance
% $\calW$. 

We now define two quantities depending only on $S$ (and importantly,
not on $h$), which will be useful in controlling the expectation and 
variance of $Y$.  The first quantity is an upper bound on $\Var[Y]$:
$$\varest \defeq \sum_{C_1 \sim_{S} C_2} \calW(C_1) \calW(C_2).$$
The second quantity is a lower bound on $\E[Y]$:
$$\meanest \defeq \frac{1}{4}\cdot \sum_{C \in \Act(S)} \calW(C).$$
%
% Again, an upper bound on the $\Var[Y]$ is given by
% We now define two quantities depending only on $S$ (and importantly,
% not on $h$), which will be useful in controlling the expectation and 
% variance of $Y$.  The first quantity is an upper bound on $\Var[Y]$:
% $\varest \defeq \sum_{C_1 \sim_{S} C_2} \calW(C_1) \calW(C_2).$$
% However, now the lower bound on $\E[Y]$ is given by:
% $$\meanest \defeq \frac{1}{4}\cdot \sum_{C \in \Act(S)} \calW(C).$$
%\Sknote{This 1/4 is correct? We should see how the next statement gets affected by the 1/4.}
%The only situation where we will use $\meanest$ is when
%$p: V \setminus S \to \{0,1\}$ is chosen to maximize
%$\E[Y]$; 
%
%
\begin{lemma}
\label{lemma:max-sat:uvar_lmean_relation}
Let $S \subseteq V$ be a subset of variables and $h: S \to \{0,1\}$ be an arbitrary partial assignment to $S.$ Let $p, Y, \varest, \meanest$ be as above.
\begin{enumerate}
\item If $\varest \le \delta_0 \epsilon_0^2
  \cdot \meanest^2,$ then $\Pr[Y < (1-\epsilon_0) \E[Y] ] < \delta_0$.
\item If $\varest \ge \delta_0\epsilon_0^2 \cdot \meanest^2 $, then there exists $v \in V\setminus S$ such that 
$$\activedeg_S(v, \calW) \geq \frac{1}{64}\epsilon_0^2\delta_0 \cdot \activedeg_{S}( \calW).$$
\end{enumerate}
\end{lemma}

We defer the formal proof to the appendix. The crux is that
independent of the assignment $h: S \to \{0,1\}$, $\E[Y] \geq
\meanest$ and $\Var(Y) \leq \varest$ (this crucially requires that the
rounding is independent and \emph{smooth}, \emph{i.e.}, $p(v) \in
[\nfrac{1}{4}, \nfrac{3}{4}]$ for all $v$; this is why we end up using
Trevisan's rounding procedure in Theorem~\ref{thm:sattrev}).  The
first part is then a simple application of the Chebyshev
inequality. For the second part, we use the assumption that $\varest$
is large, to deduce that there exists a constraint $C$ such that the
total weight of constraints that share a variable from $V \setminus S$
with $C,$ \emph{i.e.}, $\sum_{C_2 \sim_S C} \calW(C_2),$ is large. It
then follows that at least one variable $v \in C$ must have large
activedegree given $S.$

% This lemma is nearly identical to
% Lemma~\ref{lemma:max-cut:uvar_lmean_relation}, and we omit the proof.
 
%Let $S \subseteq V$. We say a contraint $C \in \calC$ is active given
%$S$ if $C$ depends on some variable from $V\setminus S$.  We denote by
%$\Act(S)$ the set of constraints from $\calC$ which are active given
%$S$.  For two constraints $C_1,C_2 \in \calC,$ we say $C_1 \sim_S C_2$
%if they share a variable in $V \setminus S$.
%
%Define the active degree of a variable $v$ given $S$ by:
%$$\activedeg_S(v, \calW) \defeq \sum_{ C \in \Act(S), C \owns v} \calW(C).$$
%
%We then define the active degree of the whole instance $\calW$ given $S$:
%$$\activedeg_S(\calW) \defeq \sum_{v \in V\setminus S} \activedeg_{S}(v,
%\calW).$$
%
%Given a set of variables $S \subseteq V,$ and a partial assignment $f:
%S \to \{0,1\}$, we define
%$$\val(f,\calW,S) \defeq  \sum_{\substack{C \in \calC \\  C \notin \Act(S)}} \calW(C) \cdot C(f).$$
%Thus, for a total assignment $g: V \to \{0,1\}$, we have $\val(g,\calW) =
%\val(g,\calW,V).$ Moreover, we have the equality:
%$$\val(g,\calW) - \val(g|_S,\calW,S) = \sum_{C \in \Act(S)}\calW(C) \cdot C(g).$$
%



%
%
%Let $S \subseteq V$ be a subset of variables, and let $h: S \to
%\{0,1\}$ be an arbitrary partial assignment to $S$.  Let $p: V \to
%[0,1]$ be such that $p|_S = h$.  For each $v \in V$, pick $g(v) \in
%\{0, 1\}$ independently with $\E[g(v)] = p(v)$. Note that $g|_S = h$
%independent of the random choices.
%
%Define the random variable
%$$Y \defeq \val(g,\calW) - \val(g|_S,\calW,S) = \sum_{C \in \Act(S)} \calW(C)\cdot C(g).$$
%The random variable $Y$ measures the contribution of active
%constraints to the instance specified by $\calW.$  Let $\mu = \E[Y]$.
%
%We now define two quantities depending only on $S$ (and importantly,
%not on $h$), which will be useful in controlling the variance and
%expectation of $Y$.  The first quantity is an upper bound on $\Var[Y]$
%(and does not depend on $h$):
%$$\varest \defeq \sum_{\substack{C_1 \sim_S C_2 \\ C_1, C_2 \in \Act(S)}} \calW(C_1) \calW(C_2).$$
%The second quantity is supposed to be a lower bound
%on $\E[Y]$ (again independent of $h$),
%$$\meanest \defeq \alpha \cdot \sum_{C \in \Act(S)} \calW(C),$$
%where $\alpha$ is a constant specifying the approximation ratio we
%would like to achieve.

% Similar to the $\maxcut$ case, we have the following lemma for $\maxsat.$ Since, the proof is almost identical, we omit the proof here.
% \begin{lemma}
% \label{lemma:uvar_lmean_relation}
% Let $S, Y, \varest, \meanest$ be as in the notation section.
% Suppose $\E[Y] \geq \meanest$.
% \begin{enumerate}
% \item If $\varest \le \delta_0 \epsilon_0^2 \cdot \meanest^2,$ then $\Pr[Y <  (1-\epsilon_0) \E[Y] ] < \delta_0$.
% \item If $\varest \ge \delta_0\epsilon_0^2 \cdot \meanest^2 $, then there exists $v \in V\setminus S$ such that 
% $$\activedeg_S(v, \calW) \geq \frac{\alpha^2}{4}\epsilon_0^2\delta_0 \cdot \activedeg_{S}( \calW).$$
% \end{enumerate}
% \end{lemma}
%\begin{proof}
%We first prove that $\Var(Y) \leq \varest$.
%Recall that the indicator variable $C(g)$ denotes whether the
%constraint $C$ is satisfied by the assignment $g$,
%and note that:
%$$Y = \sum_{C \in \Act(S)} \calW(S) \cdot C(g).$$
%Thus, the variance of $Y$ is given by
%\begin{align*}
%  \Var(Y) &= \sum_{C_{1}, C_{2}\in \Act(S)} \calW(C_1) \calW(C_2) \cdot ( \E[C_1(g)C_2(g)] - \E[C_1(g)]\E[C_2(g)] )\\
%&\leq \sum_{ \substack{C_{1} \sim_S C_{2} \\ C_{1}, C_{2} \in \Act(S)}} \calW(C_1) \calW(C_2) \\
%&= \varest,
%\end{align*}
%where the inequality holds because $\E[C_1(g)C_2(g)] -
%\E[C_1(g)]\E[C_2(g)] \le 1$ for all $C_{1}, C_{2},$ and
%$\E[C_1(g)C_2(g)] - \E[C_1(g)]\E[C_2(g)] = 0$ unless $C_{1} \sim_S
%C_{2}$ because the rounding is performed independently for all the
%variables.
%
%
%If we are in case 1 of the lemma, we have by Chebyshev's inequality:
%$$\Pr[Y <  (1-\epsilon_0) \mu ] \leq \frac{\Var(Y)}{\epsilon_0^2 \mu^2} \leq \frac{\varest}{\epsilon_0^2 \meanest^2} \leq \delta_0.$$
%Otherwise, we have:
%\begin{align*}
%  \delta_0 \epsilon_0^2 \meanest^2 &< \varest\\
%  &=\sum_{ \substack{C_{1} \sim_S C_{2} \\ C_{1}, C_{2} \in \Act(S)}}
%  \calW(C_1) \calW(C_2) \\
%  & \leq \sum_{C_{1} \in \Act(S) } \calW(C_1) \left. \sum_{
%      \substack{C_{2} \sim_S C_{1} \\  C_{2} \in \Act(S)}} \calW(C_2)   \right. \\
%  & \leq \left( \sum_{C_{1} \in \Act(S)} \calW(C_1) \right) \cdot
%  \max_{C \in \Act(S)}\left. \sum_{ \substack{C_{2} \sim_S C \\  C_{2}\in \Act(S)}} \calW(C_2)   \right. \\
%  & \leq \frac{1}{\alpha} \meanest \cdot \max_{C \in \Act(S)
%  }\left. \sum_{ \substack{C_{2} \sim_S C \\ C_{2} \in
%        \Act(S)}} \calW(C_2)\right. .
%\end{align*}
%Thus, there exists $C \in \calC$ such that:
%$$\left. \sum_{ \substack{C_{2} \sim_S C \\ C_{2}\in
%      \Act(S)}} \calW(C_2) \right. \geq \frac{1}{\alpha}\delta_0
%\epsilon_0^2 \cdot \meanest \geq \frac{1}{2}\delta_0 \epsilon_0^2
%\cdot \activedeg_S(\calW),$$ where we used the fact that $\meanest =
%\alpha \cdot ( \sum_{C \in \Act(S)} \calW(C) ) \geq \frac{\alpha}{2}
%\cdot \activedeg_S(\calW)$, since each constraint involves at most 2
%variables.
%
%Finally, if $U$ is the set of vertices in $V \setminus S$ on which
%$C_{j_1}$ depends (note that $|U| \leq 2$), then the LHS of the above
%inequality is at most $\sum_{u \in U} \activedeg_{S}(u, \calW)$.  Thus
%there is some $u \in V \setminus S$ with:
%$$\activedeg_{S}(u, \calW) \geq \frac{1}{4}\delta_0 \epsilon_0^2 \cdot \activedeg_S(\calW).$$
%\end{proof}


\subsection{Algorithm for Simultaneous \maxsat}
In Figure~\ref{fig:weighted-maxsat}, we give our algorithm for
simultaneous \maxsat. The input to the algorithm consists of an
integer $k \ge 1,$ $\eps > 0$, and $k$ instances of \maxsat, specified
by weight functions $\calW_1,\ldots,\calW_k,$ and target objective
values $c_1,\ldots,c_\ell.$
%
\begin{figure*}
\begin{tabularx}{\textwidth}{|X|}
\hline
\vspace{0mm}
{\bf Input}: $k$ instances of \maxsat $\calW_1,\ldots,\calW_k$ on the
variable set $V,$ target objective values $c_1,\ldots,c_k,$ and $\eps > 0$. \\
{\bf Output}: An assignment to $V.$ \\
{\bf Parameters:} $\delta_0 = \frac{1}{10k}$, $\epsilon_0 =
\frac{\eps}{2}$, $\gamma=\frac{\eps_0^2\delta_0}{64}$, $t =
\frac{2k}{\gamma}\cdot\log\left( \frac{11}{\gamma}\right).$
\begin{enumerate}[itemsep=0mm, label=\arabic*.]
\item Initialize $S \leftarrow \emptyset$.
\item For each instance $\ell \in [k]$, initialize $\cnt_\ell
  \leftarrow 0$ and $\flag_\ell \leftarrow \true.$
\item Repeat the following until for every $\ell \in [k]$, either $\flag_\ell = \false$ or
$\cnt_\ell  = t$:
\label{item:alg:max-sat:loop}
\begin{enumerate}
\item For each $\ell \in [k]$, compute
$\varest_\ell = \sum_{C_1 \sim_S C_2} \calW_\ell(C_1) \calW_\ell(C_2).$
\item For each $\ell \in [k],$ compute
$\meanest_\ell = \frac{1}{4} \sum_{C \in \Act(S)} \calW_\ell(C).$
\item For each $\ell \in [k],$ if $\varest_\ell \geq \delta_0
  \epsilon_0^2 \cdot \meanest_\ell^2 $, then set $\flag_\ell = \true$,
  else set $\flag_\ell = \false$.
\item Choose any $\ell \in [k]$, such that
$\cnt_\ell < t$ AND $\flag_\ell = \true$ (if any):
\label{item:alg:max-sat:high-var}
\begin{enumerate}
\item
\label{item:findv}
Find a variable $v \in V$ such that $\activedeg_S(v, \calW_\ell)
  \geq \gamma \cdot
  \activedeg_S(\calW_\ell).$ %If no such variable exists, output \fail.
\item Set $S \leftarrow S \cup \{v\}.$ We say that $v$ was brought
  into $S$ because of instance $\ell$.
\item Set $\cnt_\ell \leftarrow \cnt_\ell + 1$.
\end{enumerate}
\end{enumerate}
\item For each partial assignment $h_0: S \to \{0,1\}$:
\label{item:alg:max-sat:partial}
\begin{enumerate}
\item 
\label{item:alg:max-sat:lp}
If there is a feasible solution $\vec{t}, \vec{z}$ to the LP in
Figure~\ref{fig:max2sat-lp2}, set $p = \smooth(\vec{t})$.
If not, return to Step~\ref{item:alg:max-sat:partial} and proceed to the next $h_0$.
\item 
  \label{item:alg:max-sat:random}
Define $g: V\setminus S \to \{0,1\}$ by independently sampling
$g(v) \in \{0,1\}$ with $\E[g(v)] = p(v),$ for each $v \in V\setminus S.$
\item 
\label{item:alg:max-sat:innerh}
For each $h: S \to \{0,1\},$ compute $\out_{h,g} = \min_{\ell \in [k]}
\frac{\val(h \cup g,\calW_\ell)}{c_\ell}$. If $c_\ell = 0$ for some
$\ell \in [k],$ we interpret $\frac{\val(h\cup g,\calW_\ell)}{c_\ell}$ as
$+\infty.$
\end{enumerate}
\item Output the largest $\out_{h,g}$ seen, and the assignment $h \cup g$.
\end{enumerate}
\\ 
\hline
\end{tabularx}
\caption{Algorithm {\algowsat} for approximating weighted simultaneous
  \maxsat}
  \label{fig:weighted-maxsat}
\end{figure*}


% \begin{figure*}
% \begin{tabularx}{\textwidth}{|X|}
% \hline
% \vspace{-5mm}
% \begin{center}
% \[\begin{array}{rllr}
%  \sum_{C\in \calC} \calW_\ell(C)\cdot z_C & \geq & c_\ell & \forall \ell\in [k]\\  %(1-\nfrac{\eps}{2})\cdot
%  \sum_{v\in C^{+}} y_v + \sum_{v\in C^{-}} (1-y_v) &\geq & z_C & \forall C\in \calC\\
%  1\geq z_C &\geq & 0 & \forall C\in \calC\\
%  1\geq y_v &\geq & 0 & \forall v \in V\setminus S\\
%  y_v & = & h_0(v) & \forall v \in S
% \end{array}\]
% \end{center}
% \vspace{-30pt}
% \\
% \hline
% \end{tabularx}
% \caption{Linear Program $\LLsat(h_0)$, for a given partial assignment $h_0: S \to \{0,1\}$}
%   \label{fig:maxsat-lp}
% \end{figure*}
% \Ssnote{remove $\lp_\rho. Change y_v$. Break up into LPs}


\begin{figure*}
\begin{tabularx}{\textwidth}{|X|}
\hline
\vspace{-9mm}
\begin{center}
\[\begin{array}{rrllr}
 \sum_{v\in C^{+}} t_v + \sum_{v\in C^{-}} (1-t_v) &\geq & z_C & \forall C\in \calC\\
 1\geq z_C &\geq & 0 & \forall C\in \calC\\
 1\geq t_v &\geq & 0 & \forall v \in V\setminus S\\
 t_v & = & h_0(v) & \forall v \in S \\
\end{array}\]
\vspace{-24pt}
\end{center}
\\
\hline
\end{tabularx}
\caption{Linear program $\LLsat_1(h_0),$ for a given partial
  assignment $h_0: S \to \{0,1\}$}
  \label{fig:max2sat-lp1}
\end{figure*}


\begin{figure*}
\begin{tabularx}{\textwidth}{|X|}
\hline
\vspace{-9mm}
\begin{center}
\[\begin{array}{rrllr}
\sum_{C\in \calC} \calW_\ell(C)\cdot z_C  \geq c_\ell & \forall \ell\in [k]\\
\vect, \vecz  \text{ satisfy }  \LLsat_1(h_0).&
\end{array}\]
\vspace{-24pt}
\end{center}
\\
\hline
\end{tabularx}
\caption{Linear program $\LLsat_2(h_0)$ for a given partial assignment
  $h_0: S \to \{0,1\}$}
  \label{fig:max2sat-lp2}
\end{figure*}

\subsection{Analysis of Algorithm {\algowsat}}
\label{sec:max-sat:analysis}
%\Sknote{Removed the lemma .. made it just text.}
%
It is easy to see that the algorithm always terminates in polynomial
time. Part 2 of Lemma~\ref{lemma:max-sat:uvar_lmean_relation} implies
that that Step~\ref{item:findv} always succeeds in finding a variable
$v$. Next, we note that Step~\ref{item:alg:max-sat:loop} always
terminates. Indeed, whenever we find an instance $\ell \in [k]$ in
Step~\ref{item:alg:max-sat:high-var} such that $\cnt_\ell < t$ and
$\flag_\ell = \true,$ we increment $\cnt_\ell.$ This can happen only
$tk$ times before the condition $\cnt_\ell < t$ fails for all $\ell
\in [k].$ Thus the loop must terminate within $tk$ iterations.

Let $S^\star$ denote the final set $S$ that we get at the end of
Step~\ref{item:alg:max-sat:loop} of {\algowsat}. To analyze the
approximation guarantee of the algorithm, we classify instances
according to how many vertices were brought into $S^\star$ because of
them.
%
\begin{definition}[Low and high variance instances]
At the completion of Step~\ref{item:alg:max-sat:high-var} in Algorithm
{\algowsat}, if $\ell \in [k]$ satisfies $\cnt_\ell = t$, we call
instance $\ell$ a {\em high variance} instance.  Otherwise we call
instance $\ell$ a \emph{low variance} instance.
\end{definition}
%

% \Sknote{Let us do the perturbation to $h^\star \cup g$, as we do later
%   in the more advanced algorithms.}

% \Sknote{Maybe we should define $S^\star$ to be the set $S$ at the end
%   of the algorithm ? This might make notation much much better,
%   because we keep talking about earlier $S$'s from the middle of the
%   algorithm}

At a high level, the analysis will go as follows: First we analyze
what happens when we give the optimal assignment to $S^\star$ in
Step~\ref{item:alg:max-sat:partial} For low variance instances, the
fraction of the constraints staisfied by the LP rounding will
concentrate around its expectation, and will give the desired
approximation. For every high variance instance, we will see that many
of its ``heavy-weight" vertices were brought into $S^\star$, and we
will use this to argue that we can satisfy a large fraction of the
constraints from these high variance instances by suitably perturbing
the optimal assignment to $S^\star$ to these ``heavy-weight''
vertices. It is crucial that this perturbation is carried out without
significantly affecting the value of the low variance instances.

Let $f^\star: V \to \{0,1\}$ be an assignment such that $\val(f^\star,
\calW_\ell) \geq c_\ell$ for each $\ell$. Let $h^\star = f^\star
|_{S^\star}$. Claim 1 from Theorem~\ref{thm:sattrev} implies that
$\LLsat_2(h^\star)$ has a feasible solution.
% We first show that for low variance instances, when $g :
% V \setminus S^\star \to \{0,1\}$ is picked uniformly at random, then
% $\val(h^\star \cup g, \calW_\ell)$ is at least $\left(\nfrac{1}{2} -
%   \nfrac{\epsilon}{2}\right) \cdot c_\ell$ with high probability.
% \Sknote{Need to write this lemma .. basically take the low variance
% analysis from the proof of the theorem.}
For low variance instances, by combining Theorem~\ref{thm:sattrev} and
Lemma~\ref{lemma:max-sat:uvar_lmean_relation}, we show that
$\val(h^\star \cup g, \calW_\ell)$ is at least $\left(\nfrac{3}{4} -
  \nfrac{\epsilon}{2}\right) \cdot c_\ell$ with high probability.
\begin{lemma}
\label{lemma:maxsat:lowvariance}
Let $\ell \in [k]$ be any low variance instance. 
Let $\vec{t}, \vec{z}$ be a feasible solution to $\LLsat_2(h^\star)$.
Let $p = \smooth(\vec{t})$. 
Let $g : V \setminus S^\star \to \{0,1\}$ be such that each $g(v)$ is
sampled independently with $\E[g(v)] = p(v)$. Then the assignment
$h^\star \cup g$ satisfies:
$$ \Pr_{g} \left[ \val(h^\star
\cup g,\calW_\ell) \geq
  (\nicefrac{3}{4}-\nicefrac{\epsilon}{2})\cdot c_\ell \right] \geq 1-\delta_0.$$
\end{lemma}
\begin{proof}
  Since $\ell$ is a {\em low variance} instance, $\flag_{\ell} =
  \false$ when the algorithm terminates. Thus $\varest_\ell <
  \delta_0\epsilon_0^2 \cdot \meanest_\ell^2$.  Let $g: V \to \{0,1\}$
  be the random assignment picked in
  Step~\ref{item:alg:max-sat:random}. Define the random
  variable \[Y_\ell \defeq \val(h^\star \cup g,\calW_\ell) -
  \val(h^\star,\calW_\ell).\]

By Lemma~\ref{lemma:max-sat:uvar_lmean_relation}, we know that with probability
  at least $1-\delta_0,$ we have $ Y_\ell \ge (1- \epsilon_0) \E[Y_\ell].$
  Thus, with probability at least $1-\delta_0,$ we have,
\begin{align*}
  \val(h^\star\cup g,\calW_\ell) & = \val(h^\star,\calW_\ell) + Y_\ell \ge
  \val(h^\star,\calW_\ell)  + (1- \epsilon_0) \E[Y_\ell]\\
  & \ge (1-\epsilon_0) \cdot \av[\val(h^\star,\calW_\ell) + Y_\ell] =
  (1-\epsilon_0)\cdot \av[\val(h^\star\cup g,W_\ell)] \\
& \ge \nfrac{3}{4}\cdot (1-\epsilon_0) \cdot \sum_{C \in \calC} \calW_\ell(C) z_C \ge
  \left(\nfrac{3}{4} - \nfrac{\eps}{2}\right) \cdot c_\ell ,
\end{align*}
where the last two inequalities follow from Claim 2 in
Theorem~\ref{thm:sattrev} and the constraints in $\LLsat_2$
respectively.
%\Anote{Used $\eps_0 = \eps$}
\end{proof}

Now we analyze the high variance instances. We prove the following
lemma that proves that at the end of the algorithm, the activedegree
of high variance instances is small, and is dominated by the
activedegree of any variable that was included in $S$ ``early on".
\begin{lemma}
\label{lemma:earlyvariables}
%Let $\gamma= \frac{\epsilon_0^2\delta_0}{16}.$
For all high variance instances $\ell\in [k],$ we have 
\begin{enumerate}
\item $\activedeg_{S^\star}(\calW_\ell) \leq 2(1-\gamma)^t.$ 
\item For each of the first $\nicefrac{t}{2}$ variables that were brought
  inside $S^\star$ because of instance $\ell,$ the total weight of constraints
  incident on each of that variable and totally contained inside $S^\star$ is at
  least $10\cdot\activedeg_{S^\star}(\calW_\ell).$
\end{enumerate}
\end{lemma}
The proof of the lemma is quite simple and is deferred to the
appendix. The crucial observation is that when a variable $u$ is brought
into $S$ because of an instance $\ell,$ the activedegree of $u$ is at
least a $\gamma$ fraction of the total activedegree of instance $\ell.$ Thus,
the activedegree of instance $\ell$ goes down by a multiplicative factor of
$(1-\gamma).$ This immediately implies the first part of the
lemma. For the second part, we use the fact that $t$ is large, and hence the
activedegree of early vertices must be much larger than the final
activedegree of instance $\ell$.
%\Ssnote{@Swastik: Please read this part.}

% By lemma~\ref{lemma:uvar_lmean_relation}, we know that
%   $\activedeg_{S_{u_1}}(u_1,\calW_\ell) \geq \gamma
%   \cdot\activedeg_{S_{u_1}}(\calW_\ell)$. Hence, when we bring that
%   variable into set $S$ the active degree of instance $\ell$ reduces
%   to $(1-\gamma)$ fraction of its current active degree which is at
%   most $2(1-\gamma)$. Continuing this way, we have
%   $\activedeg_{S_{u_i}}(\calW_\ell) \leq 2(1-\gamma)^{i-1}$ for all
%   $i\in [t]$. And hence $\activedeg_S(\calW_\ell) \leq (1-\gamma)^t
%   \cdot \activedeg_{\emptyset}(\calW_\ell) \le 2 (1-\gamma)^t$.

% \Ssnote{Rewrite the part below this.}
% Since $u_t$ is the last vertex that we brought inside $S$, we have $\wt(u_t) \geq \gamma\cdot\activedeg_S(\calW_\ell)$. In general, we have $\wt_{\calW_\ell}(u_i) \geq \gamma(1+\gamma)^{t-i}\cdot\activedeg_S(\calW_\ell)$. And hence, for all $i\in [t/2]$, we have $ \wt_{\calW_\ell}(u_i) \geq \gamma(1+\gamma)^{t/2}\cdot\activedeg_S(\calW_\ell)  = \frac{\gamma}{\sqrt{\delta}}\cdot\activedeg_S(\calW_\ell)$ which is at least $7\cdot\activedeg_S(\calW_\ell)$. Therefore, total weight of $u_i$ inside $S$ is at least $7\cdot\activedeg_S(\calW_\ell) - \activedeg_S(\calW_\ell)$ which is at least $6\cdot\activedeg_S(\calW_\ell)$ as required.


% \Anote{We need to define weight associated with a variable in an instance, using $\wt_{\calW_\ell}$ here}

% \Anote{Will set the expression $2(1-\gamma)^t$ later, update : I don't think we need this}


%\Sknote{ Making changes here for the new perturb algorithm. Please check}
We now describe a procedure {\sc Perturb} (see
Figure~\ref{fig:maxcut-perturb}) which takes $h^\star: S^\star \to \B$ and
$g : V \setminus S^\star \to \B$, and produces 
a new $h : S^\star \to \B$ such that
for all (low variance as well as  high variance) instances $\ell \in [k]$,
$\val(h \cup g, \calW_\ell)$ is not much smaller than $\val(h^\star \cup g, \calW_\ell)$, and 
%$$\val(h \cup g, \calW_\ell) \ge \left(1 - \frac{\epsilon}{2}\right) \cdot \val(h^\star \cup g, \calW_\ell),$$
furthermore, for all high variance instances $\ell \in [k]$, $\val(h
\cup g, \calW_\ell)$ is large. The procedure works by picking a
special variable in $S^\star$ for every { high variance} instance and
perturbing the assignment of $h^\star$ to these special variables. The
crucial feature used in the perturbation procedure, which holds for
\maxsat (but not for \maxand), is that it is possible to satisfy a
constraint by just changing one of the variables it depends on.  The
partial assignment $h$ is what we will be using to argue that
Step~\ref{item:alg:max-sat:partial} of the algorithm produces a good
Pareto approximation.  More formally, we have the following Lemma.
% \Anote{Are we repeating above things, look at
%   Lemma~\ref{lemma:maxcut_perturbationeffect} } \Sknote{ removed the
%   repetition.}
 %\Sknote { Perturb algorithm + proof of lemma should be changed. should match notation from above.}

\begin{figure*}
\begin{tabularx}{\textwidth}{|X|}
\hline
\vspace{0mm}
{\bf Input}: $h^\star: S^\star \to \B$ and
$g : V \setminus S^\star \to \B$\\
{\bf Output}: A perturbed assignment $h :  S^\star \to \{0,1\}.$ 
%
\begin{enumerate}[itemsep=0mm, label=\arabic*.]
\item Initialize $h \leftarrow h^\star.$
\item For $\ell = 1, \ldots, k$, if instance $\ell$ is a high variance
  instance case (i.e., $\cnt_\ell = t$), we pick a special variable
  $v_\ell \in S^\star$ associated to this instance as follows:
\begin{enumerate}
\item Let $B = \{ v \in V \mid \exists \ell \in [k] \mbox{ with }
  \sum_{C \in \calC, C \owns v} \calW_{\ell}(C)\cdot C(h \cup g) \geq
  \frac{\epsilon}{2k} \cdot\val(h\cup g, \calW_\ell) \}$.  Since the weight of
  each constraint is counted at most twice, we know that $|B| \leq \frac{4k^2}{\epsilon}$.
\item Let $U$ be the set consisting of the first $t/2$ variables
brought into $S^\star$ because  of instance $\ell$.
\item Since $\nfrac{t}{2} > |B|+ k$, there exists some $u \in U$
  such that $u \not\in B \cup \{v_1, \ldots, v_{\ell-1}\}$.  We define
  $v_\ell$ to be $u$.
\item By Lemma~\ref{lemma:earlyvariables}, the total $\calW_\ell$ weight of constraints that are incident on $v_\ell$
  and only containing variables from $S^\star$ is at least
 % $\wt_{\calW_\ell}(v_\ell) \geq
  $10\cdot\activedeg_{S^\star}(\calW_\ell)$. We update $h$ by 
setting $h(v_\ell)$ to be that value from $\{0,1\}$
such that at least half of the $\calW_\ell$ weight of these constraints is
  satisfied.
\end{enumerate}
\item Return the assignment $h.$
%%\vspace{-3mm}
\end{enumerate}
% \Anote{ Shall we call the final $f|_S$ with some different name, as we
%   are not using the notation $f|_S$ in the later sections. Also, $f$
%   seems more general name for this special assignment}
\\
\hline
\end{tabularx}
\caption{Procedure {\sc Perturb} for perturbing the optimal
  assignment}
  \label{fig:maxcut-perturb}
\end{figure*}

\begin{lemma}
\label{lemma:maxcut_perturbationeffect} 
For the assignment $h$ obtained from Procedure {\sc Perturb} (see
Figure~\ref{fig:maxcut-perturb}), for each $\ell\in [k]$, $\val(h\cup
g,\calW_\ell) \geq (1-\nicefrac{\epsilon}{2}) \cdot \val(h^\star \cup
g, \calW_\ell)$. Furthermore, for each {\em high variance} instance
$\calW_\ell$, $\val(h\cup g,\calW_\ell) \geq
4 \cdot \activedeg_{S^\star}(\calW_\ell).$
\end{lemma}
\begin{proof}
  Consider the special variable $v_\ell$ that we choose for {\em high
    variance} instance $\ell \in [k]$. Since $v_\ell \notin B,$ the
  constraints incident on $v_\ell$ only contribute at most a
  $\nfrac{\eps}{2k}$ fraction of the objective value in each
  instance. 
  % all variables $v$ such that if we change the value of $v$ given by
  % $h\cup g$ then it reduces the objective value of some instance by at
  % least $\frac{\epsilon}{2k}$ fraction of it's current value. Since
  % $v_\ell$ is not present in $B$, 
  Thus, changing the assignment $v_\ell$ can reduce the value of any
  instance by at most a $\frac{\epsilon}{2k}$ fraction of their
  current objective value. Also, we pick different special variables
  for each {\em high variance} instance. Hence, the total effect of
  these perturbations on any instance is that it reduces the objective
  value (given by $h^\star \cup g$) by at most $1 - (1-
  \frac{\epsilon}{2k})^k \le \frac{\epsilon}{2}$ fraction.  Hence for
  all instances $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq
  (1-\nicefrac{\epsilon}{2})\cdot\val(h^\star\cup g,\calW_\ell)$.

  For a {\em high variance instance} $\ell \in [k]$, since $v_\ell \in
  U,$ the variable $v_\ell$ must be one of the first $\nfrac{t}{2}$
  variables brought into $S^\star$ because of $\ell.$ Hence, by
  Lemma~\ref{lemma:earlyvariables} the total weight of constraints
  that are incident on $v_\ell$ and entirely contained inside
  $S^\star$ is at least
  $10\cdot\activedeg_{S^\star}(\calW_\ell)$. Hence, there is an
  assignment to $v_\ell$ that satisfies at least at least half the
  weight of these \maxsat constraints\footnote{This is not trueif they
    are \maxand constraints.} in $\ell.$ At the end of the iteration,
  when we pick an assignment to $v_\ell,$ we have $\val(h\cup g,
  \calW_\ell) \ge 5\cdot\activedeg_{S^\star}(\calW_\ell).$ Since the
  later perturbations do not affect value of this instance by more
  than $\nfrac{\epsilon}{2}$ fraction, we get that for the final
  assignment $h$, $\val(h\cup g,\calW_\ell) \ge
  (1-\nfrac{\epsilon}{2})\cdot 5 \cdot
  \activedeg_{S^\star}(\calW_\ell) \geq 4\cdot
  \activedeg_{S^\star}(\calW_\ell).$
%  Since the total weight of constraints incident on $V \setminus S$ is
%  bounded by $\activedeg_{S^\star}(\calW_\ell),$ we get $\val(h, \calW_\ell)
%  \ge 3\cdot \activedeg_{S^\star}(\calW_\ell).$
\end{proof}


Given all this, we now show that with high probability the algorithm
finds an assignment that satisfies, for each $\ell \in [k]$, at least
$(\nfrac{3}{4}-\epsilon)\cdot c_\ell$ weight from instance
$\calW_\ell$.
%
%
\begin{theorem}
\label{thm:max-sat}
Suppose we're given $\eps \in (0,\nfrac{2}{5}],$ $k$ simultaneous
\maxsat instances $\calW_1, \ldots, \calW_\ell$ on $n$ variables, and
target objective value $c_1, \ldots,c_k$ with the guarantee that there
exists an assignment $f^\star$ such that for each $\ell \in [k],$ we
have $\val( f^\star, \calW_\ell) \ge c_\ell.$ Then, the algorithm {\algowsat} runs in time $\exp(\nfrac{k^3}{\eps^2}\log
(\nfrac{k}{\eps^2}))\cdot\poly(n),$ and with probability at least
$0.9,$ outputs an assignment $f$ such that for each $\ell \in [k],$ we
have, $\val(f, \calW_\ell) \ge \left( \nfrac{3}{4} -\epsilon\right)
\cdot c_\ell.$ 
\end{theorem}
\begin{proof}
  Consider the iteration of Step~\ref{item:alg:max-sat:partial} of the
  algorithm when $h_0$ is taken to equal $h^\star$. Then, by Part 1 of
  Theorem~\ref{thm:sattrev}, the LP in Step~\ref{item:alg:max-sat:lp}
  will be feasible (this uses the fact that $\val(f^\star, \calW_\ell)
  \geq c_\ell$ for each $\ell$).


  By Lemma~\ref{lemma:maxsat:lowvariance} and a union bound, with
  probability at least $1 -k\delta_0 > 0.9$, over the choice of $g$,
  we have that for {\em every} low variance instance $\ell \in [k]$,
  $\val(h^\star \cup g, \calW_\ell) \geq (\nfrac{3}{4} -
  \nfrac{\epsilon}{2}) \cdot c_{\ell}$. Henceforth we assume that the
  assignment $g$ sampled in Step~\ref{item:alg:max-sat:random} of the
  algorithm is such that this event occurs. Let $h$ be the output of
  the procedure {\sc Perturb} given in Figure~\ref{fig:maxcut-perturb}
  for the input $h^\star$ and $g.$
% \Anote{Should we name for this special g and h?}.
  By Lemma~\ref{lemma:maxcut_perturbationeffect}, $h$ satisfies
\begin{enumerate}
\item\label{item:max-sat:proof:guarantees:1} For every instance $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq (1-\nfrac{\eps}{2})\cdot \val(h^\star\cup g,\calW_\ell).$
\item \label{item:max-sat:proof:guarantees:2}For every high variance
  instance $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq
 4 \cdot  \activedeg_{S^\star}(\calW_\ell).$
\end{enumerate}
%Since we are trying all assignment to $S^\star$, we will be 
We now show that the desired Pareto approximation behavior is achieved
when $h$ is considered as the partial assignment in
Step~\ref{item:alg:max-sat:innerh} of the algorithm. We analyze the
guarantee for low and high variance instances separately.




% By Lemma~\ref{item:alg:max-sat:random} and a union bound, with probability at least
% $1 - k \delta_0 > 0.9$, the $g$ chosen in Step~\ref{ } will be such that for every low variance 
% instance $\ell \in [k]$, we have $\val(h^\star \cup g, \calW_\ell) \geq 
% (\nfrac{3}{4} - \nfrac{\epsilon}{2}) \cdot c_{\ell}$. 

% Henceforth we assume
% this happens.

% Now let $h$ be the output of the procedure  {\sc Perturb}~\ref{fig:maxcut-perturb} when we feed it $h^\star$ and $g$\Anote{Should we name for this special g and h?}. By Lemma~\ref{lemma:maxcut_perturbationeffect}, it satisfies
% \begin{enumerate}
% \item\label{item:maxsat:proof:guarantees:1} For every instance $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq (1-\nfrac{\eps}{2})\cdot \val(h^\star\cup g,\calW_\ell)$
% \item \label{item:maxsat:proof:guarantees:2}For every high variance instance $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq 4 \cdot \activedeg_{S^\star}(\calW_\ell)$
% \end{enumerate}
%Since we are trying all assignment to $S^\star$, we will be 
% We now show that the desired Pareto approximation behavior is achieved When this $h$ is considered in Step~\ref{item:innerh} of the algorithm. We analyze the guarantee for low and high variance instances separately.
% when we consider this perturbed assignment in Step~\ref{item:alg:max-cut:partial}. 

For any {\em low variance} instance $\ell \in [k],$ from
property~\ref{item:max-sat:proof:guarantees:1} above, we have
$\val(h\cup g,\calW_\ell) \geq (1-\nfrac{\eps}{2})\cdot
\val(h^\star\cup g,\calW_\ell)$. Since we know that $\val(h^\star \cup
g, \calW_\ell) \geq (\nfrac{3}{4}-\nfrac{\eps}{2})\cdot c_\ell$, we
have $\val(h\cup g,\calW_\ell) \geq (\nfrac{3}{4}-\eps)\cdot c_\ell$.

% Consider a {low variance} instance $\ell$, if any. From property~\ref{item:maxsat:proof:guarantees:1} above, we have $\val(h\cup g,\calW_\ell) \geq (1-\nfrac{\eps}{2})\cdot \val(h^\star\cup g,\calW_\ell)$. Since we know that $\val(h^\star \cup g, \calW_\ell) \geq (\nfrac{3}{4}-\nfrac{\eps}{2})\cdot c_\ell$, we have  $\val(h\cup g,\calW_\ell) \geq (\nfrac{3}{4}-\eps)\cdot c_\ell$.


For every high variance instance $\ell \in [k],$ since $h^\star =
f^\star|_{S^\star},$ for any $g$ we must have,
\[\val(h^\star \cup g, \calW_\ell) \ge \val(f^\star, \calW_\ell) -
\activedeg_{S^\star}(\calW_\ell) \ge c_\ell - \activedeg_{S^\star}(\calW_\ell) .\]
Combining this with properties~\ref{item:max-sat:proof:guarantees:1}
and \ref{item:max-sat:proof:guarantees:2} above, we get,
\begin{align*}
\val(h \cup g, \calW_\ell) &\ge \left( 1 - \nfrac{\epsilon}{2}
\right) \cdot \max\{c_\ell - \activedeg_{S^\star}(\calW_\ell), 4 \cdot
\activedeg_{S^\star}(\calW_\ell)\} \\
&\ge \left( \nfrac{3}{4} - \epsilon \right) \cdot c_\ell.
\end{align*}

Thus, for all instances $\ell \in [k]$, we get $\val(h \cup g) \ge
\left(\nfrac{3}{4}-\eps\right) \cdot c_{\ell}.$ Since we are taking
the best assignment $h\cup g$ at the end of the algorithm {\algowsat}, the theorem follows.
% For every high variance instance $\ell \in
% [k],$ since $h^\star = f^\star|_{S^\star},$
% \[\val(h^\star \cup g, \calW_\ell) \ge \val(f^\star, \calW_\ell) -
% \activedeg_{S^\star}(\calW_\ell) \ge c_\ell - \activedeg_{S^\star}(\calW_\ell) .\]
% Combining this with properties~\ref{item:maxsat:proof:guarantees:1}
% and \ref{item:maxsat:proof:guarantees:2} above, we get,
% \begin{align*}
% \val(h \cup g, \calW_\ell) &\ge \left( 1 - \nfrac{\epsilon}{2}
% \right) \cdot \max\{c_\ell - \activedeg_{S^\star}(\calW_\ell), 4\cdot \activedeg_{S^\star}(\calW_\ell)\} \\
% &\ge \left( \nfrac{3}{4} - \epsilon \right) \cdot c_\ell.
% \end{align*}
%
% Thus, for all instances $\ell \in [k]$, we get $\val(h \cup g) \ge
% \left(\nfrac{3}{4}-\eps\right) \cdot c_{\ell}.$
%
% Since we are taking the best assignment $h\cup g$ at the end of the algorithm {\sc WeightedMC}, the theorem follows.
% \Sknote{ Should go through the above and change the name of MAXCUT to MAXSAT.
% Also remove "weighted" from everywhere. Note that to save
% repetition, we are using the perturbation procedure +  the
% perturbation lemma from MAXCUT.}

{\bf Running time : } 
Running time of the algorithm is $2^{O(kt)}\cdot\poly(n)$ which is $\exp(\nfrac{k^3}{\eps^2}\log (\nfrac{k}{\eps^2}))\cdot\poly(n)$.
\Ssnote{Can we do a more careful analysis of the running time?}
\end{proof}

%Observe that \algowsat is identical to {\sc WeightedMC},
%except that the random assignment $g$ in
%Step~\ref{item:alg:max-sat:random} has a distribution that is now
%determined by using an linear program. Thus, we will use the notation
%and several lemmas from Section~\ref{sec:max-cut:analysis}.


%We use the same
%procedure {\sc Perturb} (see Figure~\ref{fig:maxcut-perturb} to obtain
%an assignment $f$ that specifies the partial assignment $h$ we will be
%interested in for
%Step~\ref{item:alg:max-sat:partial}. Lemma~\ref{lemma:maxcut_perturbationeffect}
%still holds about the perturbed solution generated.


% \begin{claim}
% \label{claim:earlyvariables}
% Let $\gamma= \frac{\epsilon_0^2\delta_0}{16}.$
% In the algorithm  \algowsat, for all  high variance instance $\ell\in [k],$ we have 
% \begin{enumerate}
% \item $\activedeg_S(\calW_\ell) \leq 2(1-\gamma)^t.$ 
% \item Consider the first $\nicefrac{t}{2}$ variables that we brought inside $S$
%   because of instance $\ell.$ For each of these variables, the total weight of constraints inside $S$ containing that variable is at least
%   $8\cdot\activedeg_S(\calW_\ell).$  
% \end{enumerate}
% \end{claim}
% \begin{proof}
% The proof of this is similar to~\ref{} and hence, we omit the proof here.
% \end{proof}

%\begin{proof}
%  Consider any {\em high variance} instance $\ell \in[k]$. Initially,
%  when $S=\emptyset,$ we have $\activedeg_\emptyset(\calW_\ell) \leq
%  2$ since the weight of every constraint is counted at most twice,
%  once for each of the at most 2 active variables in the constraint,
%  and $\sum_{C\in \calC } \calW_\ell(C)= 1$. Whenever we bring
%  variables from other instances into $S$, the active degree of any
%  variable $v \in V$ in the instance $\ell$ w.r.t. the current $S$
%  never goes up i.e. $\activedeg_{S_2}(v,\calW_\ell) \leq
%  \activedeg_{S_1}(v,\calW_\ell)$ for any $S_1 \subseteq S_2.$
%
%  Since $t$ variables were brought into $S$ because of instance
%  $\ell,$ and initially $\activedeg_{\emptyset}(\calW) \le 2,$ it
%  suffices to show that when a variable $u$ is brought into $S,$
%  $\activedeg$ goes down by a multiplicative factor of $(1-\gamma).$
%  Let $S_u$ be the set of variables in $S$ just before $u$ was
%  picked. From lemma~\ref{lemma:uvar_lmean_relation}, we know that
%  $\activedeg_{S_{u}}(u,\calW_\ell) \geq \gamma
%  \cdot\activedeg_{S_{u}}(\calW_\ell)$. Thus,
%\begin{align*}
%  \activedeg_{S_u \cup \{u\}}(\calW) & = \sum_{v \in V\setminus \{S
%    \cup
%    \{u\}\}} \activedeg_{S_u \cup \{u\}}(v, \calW) \\
%  & \le \activedeg_{S_u}(\calW) - \activedeg_{S_{u}}(u,\calW_\ell) \le
%  (1-\gamma) \activedeg_{S_u}(\calW).
%\end{align*}
%By induction, we get $\activedeg_S(\calW_\ell) \le (1-\gamma)^t
%  \cdot \activedeg_{\emptyset}(\calW_\ell) \le 2 (1-\gamma)^t$.
%
%  Let $u_1,u_2,\cdots,u_t$ be the set of variables brought into $S$
%  because of instance $\ell$ and let $S_{u_1}\subseteq
%  S_{u_2}\subseteq \cdots \subseteq S_{u_t}$ be the set of variables
%  in set $S$ just before we bring variables $u_1,u_2,\cdots,u_t$
%  respectively. From the above induction argument, we know that
%  $\activedeg_S(\calW_\ell) \le \activedeg_{S_{u_t}}(\calW_\ell) \le
%  (1-\gamma)^{t-i}\activedeg_{S_{u_t}}(\calW_\ell).$ Moreover, we know
%  that for any $i,$ we have $\activedeg_{S_{u_i}}(u_i,\calW_\ell) \geq
%  \gamma \cdot\activedeg_{S_{u_i}}(\calW_\ell).$ Hence, for any $i \in
%  \floor{t/2},$ we have \[\activedeg_{S_{u_i}}(u_i,\calW_\ell) \ge
%  \gamma (1-\gamma)^{i-t} \activedeg_S(\calW) \ge
%  \tfrac{\gamma}{(1-\gamma)^{t/2}} \cdot \activedeg_S(\calW_\ell),\]
%  which is at least $7\cdot\activedeg_S(\calW_\ell)$. Therefore, total
%  weight of constraints incident on $u_i$ and contained inside $S$ is
%  at least $7\cdot\activedeg_S(\calW_\ell) -
%  \activedeg_S(\calW_\ell),$ which is at least
%  $6\cdot\activedeg_S(\calW_\ell)$ as required.
%\end{proof}



%
% \begin{figure*}
% \begin{tabularx}{\textwidth}{|X|}
% \hline
% \vspace{0mm}
% {\bf Input}: $f^\star: V \to \{0,1\}$ be an assignment such that
% $\val(f^\star,\calW_\ell) \geq c_\ell$ for each $\ell \in [k].$ \\
% {\bf Output}: A perturbed assignment $f : V \to \{0,1\}.$ 
% %
% \begin{enumerate}[label=\arabic*.]
% \item Initialize $f \leftarrow f^\star.$
% \item For $\ell = 1, \ldots, k$, if instance $\ell$ is a high variance
%   instance case (i.e., $\cnt_\ell = t$), we pick a special variable
%   $v_\ell$ associated to this instance as follows:
% \begin{enumerate}
% \item Let $B = \{ v \in V \mid \exists \ell \in [k] \mbox{ with }
%   \sum_{C \in \calC, C \owns v} \calW_{\ell}(C)\cdot C(f) \geq
%   \frac{\epsilon}{2k} \val(f, \calW_\ell) \}$.  Since the weight of
%   each constraint is counted at most twice, once for each of the
%   variables contained in it, $|B| \leq \frac{4k^2}{\epsilon}$.
% \item Let $u_1, \ldots, u_t$ be the variables brought into $S$ because
%   of instance $\ell,$ in the order that they were picked.
% \item Since $\nfrac{t}{2} > |B|+ k$, there exists some $j \leq t/2$
%   such that $u_j \not\in B \cup \{v_1, \ldots, v_{\ell-1}\}$.  We define
%   $v_\ell$ to be $u_j$.
% \item The total weight of constraints that are incident on $v_\ell$
%   and only containing variables from $S$ is at least
%  % $\wt_{\calW_\ell}(v_\ell) \geq
%   $6\cdot\activedeg_S(\calW_\ell)$. Thus, we pick an assignment to
%   $v_\ell$ from $\{0,1\}$ such that the at least half the weight of
%   these constraints is satisfied.
% \end{enumerate}
% \vspace{-3mm}
% \end{enumerate}
% \\ 
% \hline
% \end{tabularx}
% \caption{Procedure {\sc Perturb} for perturbing the optimal
%   assignment}
%   \label{fig:maxsat-perturb}
% \end{figure*}


% \begin{claim}
% \label{claim:perturbationeffect} 
% For the assignment $f$ obtained from Procedure {\sc Perturb}, for each
% $\ell\in [k]$, $\val(f,\calW_\ell) \geq (1-\nicefrac{\epsilon}{2})
% \cdot c_\ell$. Furthermore, for each {\em high variance} instance
% $\calW_\ell$, $\val(f|_S,\calW_\ell,S) \geq
% 3\cdot\activedeg_S(\calW_\ell).$
% \end{claim}
%\begin{proof}
%  Recall that $f^\star$ is an optimal assignment. We will analyze the
%  effect of the perturbation to $f^\star$ by Procedure {\sc
%    Perturb}. Consider the special vertex $v_\ell$ that we choose for
%  {\em high variance} instance $\ell \in [k]$. $B$ is the set of all
%  variables $v$ such that if we change the value of $v$ given by $f^\star$
%  then it reduces the total weight of satisfied constraints of some
%  instance by at least $\frac{\epsilon}{2k}$ fraction of the value
%  given by $f^\star$. Since $v_\ell$ is not present in $B$, changing the
%  value of $v_\ell$ will reduce the value of other instances by at
%  most an $\frac{\epsilon}{2k}$ fraction. Also, we pick different
%  special vertices for each {\em high variance} instance. Hence, the
%  total effect of these perturbations on a specific instance is that
%  it reduces the total weight of satisfied constraints by at most
%  $\nicefrac{\epsilon}{2}$ fraction. And hence for all instances $\ell
%  \in [k]$, $\val(f,\calW_\ell) \geq (1-\nicefrac{\epsilon}{2})\opt$.
%
%  For a {\em high variance instance} $\ell \in [k]$, since $v_\ell=
%  u_j$ for some $j\in [t/2]$, we know by
%  claim~\ref{claim:earlyvariables} that the total weight of
%  constraints incident that are incident on $u_j$ and entirely
%  contained in $S$ is at least
%  $6\cdot\activedeg_S(\calW_\ell)$. Hence, there is an assignment to
%  $v_\ell$ that satisfies at least at least half the weight of these
%  constraints in $\ell.$ Since these constraints are entirely
%  contained in $S,$ we get $\val(f|_S,\calW_\ell,S) \ge 3\cdot \activedeg_S(\calW_\ell).$
%\end{proof}











%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "new-simopt"
%%% End: 



% %\section{Possibly Delete this Part}

% % \begin{lemma}
% % \label{lemma:max-sat:uvar_lmean_relation}
% % Let $S, Y, \varest, \meanest$ be as above.
% % \begin{enumerate}
% % \item If $\varest \ge \delta_0\epsilon_0^2 \cdot \meanest^2 $, then there exists $v \in V\setminus S$ such that 
% % $$\activedeg_S(v, \calW) \geq \frac{\alpha^2}{4}\epsilon_0^2\delta_0 \cdot \activedeg_{S}( \calW).$$
% % \item If $\E[Y] \geq \meanest,$ and $\varest \le \delta_0 \epsilon_0^2
% %   \cdot \meanest^2,$ then $\Pr[Y < (1-\epsilon_0) \E[Y] ] < \delta_0$.
% % \end{enumerate}
% % \end{lemma}
% % \begin{proof}
% % We first prove that $\Var(Y) \leq \varest$.
% % Recall that the indicator variable $C(h\cup g)$ denotes whether a
% % constraint $C$ is satisfied by the assignment $h\cup g$,
% % and note that:
% % $$Y = \sum_{C \in \Act(S)} \calW(S) \cdot C(h\cup g).$$
% % Thus, the variance of $Y$ is given by
% % \begin{align*}
% %   \Var(Y) &= \sum_{C_{1}, C_{2}\in \Act(S)} \calW(C_1) \calW(C_2) \cdot ( \E[C_1(h\cup g)C_2(h\cup g)] - \E[C_1(h\cup g)]\E[C_2(h\cup g)] )\\
% % %&\leq \sum_{ C_{j_1}, C_{j_2}, \text{both active given $S$}} \calW_{j_1} \calW_{j_2} ( \E[Y_{j_1} Y_{j_2}] - \E[Y_{j_1}]\E[Y_{j_2}] )\\
% % &\leq \sum_{ C_{1} \sim_{S} C_{2} } \calW(C_1) \calW(C_2) = \varest,
% % \end{align*}
% % where the inequality holds because $\E[C_1(h\cup g)C_2(h\cup g)] -
% % \E[C_1(h\cup g)]\E[C_2(h\cup g)] \le 1$ for all $C_{1}, C_{2},$ and
% % $\E[C_1(h\cup g)C_2(h\cup g)] - \E[C_1(h\cup g)]\E[C_2(h\cup g)] = 0$ unless $C_{1} \sim_{S}
% % C_{2}$ because the rounding is performed independently for all the
% % variables.

% % %\begin{align*}
% % %\E[Y] &= \E[\sum_{C_j \text{ active given $S$}} \calW_j Y_j]\\
% % %&\geq \sum_{C_j \text{ active given $S$}} \calW_j   \E[ Y_j ]\\
% % %& \geq  \frac{1}{2} \left(\sum_{C_j \text{ active given $S$}} \calW_j \right).
% % %\end{align*}

% % For the first part of the lemma, we have:
% % \begin{align*}
% %   \delta_0 \epsilon_0^2 \meanest^2 &< \varest
% %   =\sum_{ C_{1} \sim_{S} C_{2} }
% %   \calW(C_1) \calW(C_2) \\
% %   & \leq \sum_{C_{1} \in \Act(S) } \calW(C_1) \left. \sum_{
% %       C_{2} \sim_{S} C_{1}} \calW(C_2)   \right. \\
% % & \leq \left( \sum_{C_{1} \in \Act(S)} \calW(C_1) \right) \cdot
% % \max_{C \in \Act(S)}\left. \sum_{ C_{2} \sim_{S} C } \calW(C_2)   \right. \\
% % & \leq \frac{1}{\alpha} \meanest \cdot \max_{C \in \Act(S)
% % }\left. \sum_{ C_{2} \sim_{S} C }
% %   \calW(C_2)\right. .
% % \end{align*}
% % Thus, there exists a constraint $C \in \Act(S)$ such that:
% % \begin{equation}
% % \label{eq:lemma:uvar_lmean_relation:1}
% % \left. \sum_{ C_{2} \sim_{S} C} \calW(C_2) \right. \geq \alpha\cdot\delta_0
% % \epsilon_0^2 \cdot \meanest \ge \frac{\alpha^2}{2}\delta_0 \epsilon_0^2
% % \cdot \activedeg_S(\calW), 
% % \end{equation}
% % where we used the fact that $\meanest = \alpha \cdot ( \sum_{C \in
% %   \Act(S)} \calW(C) ) \geq \frac{\alpha}{2} \cdot
% % \activedeg_S(\calW)$, since we are counting the weight of a constraint at
% % most twice in the expression $\activedeg_S(\calW).$ Finally, the LHS
% % of equation~\eqref{eq:lemma:uvar_lmean_relation:1} is at most $\sum_{u
% %   \in C \cap (V \setminus S)} \activedeg_{S}(u, \calW)$.  Thus, there is some $u \in V
% % \setminus S$ with:
% % $$\activedeg_{S}(u, \calW) \geq \frac{\alpha^2}{4}\delta_0 \epsilon_0^2 \cdot \activedeg_S(\calW).$$

% % The second part of the lemma easily follows from Chebyshev's inequality:
% % $$\Pr[Y <  (1-\epsilon_0) \E[Y] ] \leq \frac{\Var(Y)}{\epsilon_0^2 (\E[Y])^2} \leq \frac{\varest}{\epsilon_0^2 \meanest^2} \leq \delta_0.$$
% % \end{proof}







% %   Let $f$ be the assignment specified by Procedure {\sc Perturb},
% %   starting with the initial assignment $f^\star : V \to \B$. We
% %   show that for the partial assignment $f|_{S}$ to the variables in
% %   $S,$ the algorithm achieves the claimed approximation guarantee. The
% %   proof of the claim for {\em high variance} instances is similar to
% %   the one in Theorem~\ref{thm:max-cut} and we will not repeat it here. We
% %   will prove the claim for {\em low variance} instances.
% % \begin{enumerate}
% %\item {\bf High variance instances:} 
% %
% %  Let $\ell\in [k]$ be a {\em high variance} instance, if any. We know
% %  by Claim~\ref{claim:perturbationeffect} that regardless of the
% %  assignment to the variables in $V\setminus S$, the weight of the
% %  satisfied constraints within $S$ will be at least
% %  $3\cdot\activedeg_S(\calW_\ell)$ weight. 
% %
% %  Consider two cases: If $\opt < 4\cdot\activedeg_S(\calW_\ell),$ then
% %  using $\val(f|_{S}, \calW_\ell,S) \ge 3\cdot\activedeg_S(\calW_\ell),$ we
% %  get regardless of the assignment to variables in $V\setminus S,$ the
% %  weight of the constraints satisfied in instance $\ell$ is at least
% %  $\nicefrac{3}{4} \cdot \opt.$
% %
% %  If $\opt \ge 4\cdot\activedeg_S(\calW_\ell),$ we know that
% %  $\val(f,\calW_\ell) \ge (1-\nicefrac{\eps}{2})\cdot\val(f^\star,\calW_\ell) \ge 
% %  (1-\eps)\cdot \opt.$ Moreover, since the total weight of the
% %  constraints that contain at least one variable from $V \setminus S$
% %  is at most $\activedeg_S(\calW_\ell),$ regardless of the assignment
% %  to variables in $V\setminus S,$ the weight of the constraints
% %  satisfied is at least
% %\[\val(f|_{S},\calW_\ell) \ge (1-\eps)\cdot\opt - \activedeg_S(\calW_\ell) \ge
% %(\nicefrac{3}{4}-\eps)\cdot \opt.\]

% \item {\bf Low variance instances: }
 
%   Let $p: V \to [0,1]$ be the LP solution for a partial assignment
%   $f|_S$ given by Step~\ref{item:alg:max-sat:lp}. Consider the
%   following solution to the LP: For every variable $v \in V,$ we let
%   $y_v$ be 1 iff the assignment $f$ sets $v$ to $\true.$ Also, for
%   every constraint $C \in \calC,$ we let $z_C = C(f).$ For this
%   solution, we obtain that the $\val(f,\calW_\ell) \ge
%   (1-\nicefrac{\eps}{2})\cdot c_\ell.$ Thus, for this partial
%   assignment $h = f|_S$, the LP is feasible. Consider a {\em low
%     variance} instance $\ell$, if any. We know that $\flag_{\ell} =
%     \false$ when the algorithm terminates. Thus $\varest_\ell <
%   \delta_0\epsilon_0^2 \cdot \meanest_\ell^2$.  Let $g: V\setminus S
%   \to \{0,1\}$ be the random assignment picked in
%   Step~\ref{item:alg:max-sat:random}. Define the random
%   variable \[Y_\ell \defeq \val(f|_S \cup g,\calW_\ell) -
%   \val(f|_S,\calW_\ell).\]

%   It was proved by Goemans and Williamson~\cite{GW-maxsat} that for
%   one \maxsat instance ($k=1$), the rounding procedure used by the
%   algorithm, \emph{i.e.}, rounding each variable independently
%   according to the probabilities $P$ provided by the LP, produces an
%   assignment $g$ such that, in expectation, $\val(f|_s \cup g , \calW_\ell) \ge
%   \frac{3}{4} \val(p, \calW_\ell).$ Since $p$ is a feasible solution
%   to the LP, we know that $\val(p, \calW_\ell) \ge
%   (1-\nfrac{\epsilon}{2}) \cdot c_\ell.$ By
%   Lemma~\ref{lemma:max-cut:uvar_lmean_relation}, we know that with probability
%   at least $1-\delta_0,$ we have $ Y_\ell \ge (1- \epsilon_0) \E[Y].$
%   Thus, with probability at least $1-\delta_0,$ we have,
% \begin{align*}
%   \val(f|_S \cup g,\calW_\ell) & = \val(f|_S,\calW_\ell) + Y_\ell \ge
%   \val(f|_S,\calW_\ell)  + (1- \epsilon_0) \E[Y]\\
%   & \ge (1-\epsilon_0) \cdot \av[\val(f|_S,\calW_\ell) + Y_\ell] =
%   (1-\epsilon_0)\cdot \av[\val(f|_S \cup g,W_\ell)] \\
% & \ge \nfrac{3}{4} \cdot (1-\eps_0) \cdot \val(p, \calW_\ell) \\
%   & \ge \nfrac{3}{4}\cdot (1-\epsilon_0) (1-\nicefrac{\eps}{2}) \cdot c_\ell \ge
%   \left(\nfrac{3}{4} - \epsilon_0 - \nicefrac{\eps}{2}\right) \cdot c_\ell = \left(\nfrac{3}{4} - \eps\right) \cdot c_\ell .
% \end{align*}
% Hence, by a union bound, with probability at least $1-k\delta_0 =
% 0.9,$ we get a $\left(\nfrac{3}{4} -\epsilon\right)$ approximate
% solution for every {\em low variance instance}.
%  % $\E[Y] \geq \frac{3}{4} Y_h$ ~\cite{GW-maxsat}
%  %  \Anote{shall we write the proof of this may be in Appendix? or this
%  %    is okay}, where $Y_h$ is an upper bound of the optimal value of
%  %  $Y$ that we get after extending assignment $f^\star|_{S}$ to $V\setminus
%  %  S$ i.e $Y_h \geq \opt$ \Anote{check if I am doing any mistakes
%  %    here}. By lemma~\ref{lemma:uvar_lmean_relation}, we thus have
%  %  $\Pr[ Y < (1- \epsilon_0) \E[Y] ] < \delta_0$. And since, changing
%  %  assignment $f^\star_{|S}$ to $f|_{S}$, as given by {\em Procedure} $1$,
%  %  reduces the value of any instance $\ell\in [k]$ by at most
%  %  $\epsilon\cdot \val(f^\star,\calW_\ell)$, we get a
%  %  $\left(\frac{3}{4}-\epsilon - \frac{3\epsilon_0}{4}\right)$
%  %  approximate solution with probability at least $(1-\delta_0)$.
% \end{enumerate}
% %{\bf Running time : } 
% %Running time of the algorithm is $2^{O(t)}\cdot\poly(n)$ which is $\exp(\nfrac{k^2}{\eps^2}\log (\nfrac{k}{\eps^2}))\cdot\poly(n)$.



% %%% Local Variables: 
% %%% mode: latex
% %%% TeX-master: "new-simopt"
% %%% End: 


==> maxcut_new.tex <==

\section{Simultaneous \maxcut}
%\Ssnote{Move these definitions to the main file}
In this section, we give our most basic simultaneous approximation algorithm, for the problem of simultaneous \maxcut.

\label{section:max-cut}


\subsection{Preliminaries}
\label{sec:notation-1}
%We fix the 2-CSP of interest, \emph{e.g.} \maxcut or \maxsat.

Let $V$ be a set of $n$ Boolean variables. Let $\calC$ denote the set of all
possible cut constraints on $V$ (thus $|\calC| = {n \choose 2}$). 
A MAXCUT instance is then described by
a weight function $\calW : \calC \to \rea_{\geq 0}$ (here $\calW(C)$ denotes
the weight of the constraint $C$). We will assume that
$\sum_{C \in \calC} \calW(C) = 1$.

%\paragraph{Constraints and $\val$}
We say $v \in C$ if the variable $v$ appears in the constraint $C$. 
Let $f: V \to \{0,1\}$ be an assignment. For a constraint $C \in
\calC,$ define $C(f)$ to be 1 if the constraint $C$ is satisfied by
the assignment $f$, and define $C(f) = 0$ otherwise
(\emph{e.g.} for a \maxcut constraint $C=(u,v)$ we
have $C(f)=1$ iff $f(u) \neq f(v)$).
Then, we have the following expression for $\val(f,\calW)$:
$$\val(f,\calW) \defeq \sum_{C \in \calC} \calW(C) \cdot C(f).$$

\subsubsection{Active Constraints}
In our algorithm, we will maintain a small set $S \subseteq V$
on which we will try all assignments by brute-force, and then
use a random assignment for $V \setminus S$. We now introduce some
notation for dealing with this.

Let $S \subseteq V$. We say a constraint $C \in \calC$ is active given
$S$ if at least one of the variables of $C$ is in $V\setminus S$.  We
denote by $\Act(S)$ the set of constraints from $\calC$ which are
active given $S$.  For two constraints $C_1,C_2 \in \calC,$ we say
$C_1 \sim_{S} C_2$ if they share a variable that is contained in $V
\setminus S$. Note that if $C_1 \sim_{S} C_2,$ then $C_1, C_2$ are
both in $\Act(S)$. For two partial assignments $f_1 : S \to \B$ and
$f_2 : V\setminus S \to \B$, let $f = f_1\cup f_2$ is an assignment
$f : V \to \B$ such that $f(x) = f_1(x)$ if $x\in S$ otherwise
$f(x) = f_2(x)$.

Define the active degree of a variable $v \in V\setminus S$ given $S$ by:
$$\activedeg_S(v, \calW) \defeq \sum_{ C \in \Act(S), C \owns v} \calW(C).$$
We then define the active degree of the whole instance $\calW$ given $S$:
$$\activedeg_S(\calW) \defeq \sum_{v \in V\setminus S} \activedeg_{S}(v,
\calW).$$
For a partial assignment $h: S \to \{0,1\}$, we define
$$\val(h,\calW) \defeq  \sum_{\substack{C \in \calC \\  C \notin \Act(S)}} \calW(C) \cdot C(h).$$
Thus, for an assignment $g: V\setminus S \to \{0,1\}$, to the
remaining set of variables, we have the equality:
$$\val(h\cup g,\calW) - \val(h,\calW) = \sum_{C \in \Act(S)}\calW(C) \cdot C(h\cup g).$$


\subsection{Random Assignments}
% \Anote{This will go into the common section, with more general claims which will work for $\maxcut$ and $\maxsat$. It is not completely similar to the CSP sections as the concept of activedegree is different there.}
We now give a sufficient
condition for the value of a \maxcut instance $\calW$ to be highly
concentrated under independent uniformly random assignment to the
variables of $V \setminus S$. When this condition does not hold,
we will get a variable of high active degree.

%We say that constraint $C_j$ is active if $\E[Y_j] \not\in \{0, 1\}$, 
%i.e., its value is not fixed.

Let $S \subseteq V$ be a subset of variables.  Let $h: S \to \{0,1\}$
be an arbitrary partial assignment to $S$.  Consider the random
assignment $g: V \setminus S \to \{0,1\}$, where for each $v \in
V\setminus S$, $g(v) \in \{0, 1\}$ is picked uniformly and
independently. Define the random variable
$$Y \defeq \val(h\cup g,\calW) - \val(h,\calW) = \sum_{C \in \Act(S)} \calW(C)\cdot C(h\cup g).$$
The random variable $Y$ measures the contribution of active
constraints to the instance $\calW$.

We now define two quantities depending only on $S$ (and importantly,
not on $h$), which will be useful in controlling the expectation and 
variance of $Y$.  The first quantity is an upper bound on $\Var[Y]$:
$$\varest \defeq \sum_{C_1 \sim_{S} C_2} \calW(C_1) \calW(C_2).$$
The second quantity is a lower bound\footnote{Here $\meanest$ is
  exactly the mean of $Y,$ but we only use the fact that it is a lower bound.
Later this added flexibility will be useful.}
on $\E[Y]$:
$$\meanest \defeq \frac{1}{2}\cdot \sum_{C \in \Act(S)} \calW(C).$$
\begin{lemma}
\label{lemma:max-cut:uvar_lmean_relation}
Let $S \subseteq V$ be a subset of variables and $h: S \to \{0,1\}$ be an arbitrary partial assignment to $S.$ Let $Y, \varest, \meanest$ be as above.
\begin{enumerate}
\item If $\varest \le \delta_0 \epsilon_0^2
  \cdot \meanest^2,$ then $\Pr[Y < (1-\epsilon_0) \E[Y] ] < \delta_0$.
\item If $\varest \ge \delta_0\epsilon_0^2 \cdot \meanest^2 $, then there exists $v \in V\setminus S$ such that 
$$\activedeg_S(v, \calW) \geq \frac{1}{16}\epsilon_0^2\delta_0 \cdot \activedeg_{S}( \calW).$$
\end{enumerate}
\end{lemma}
We defer the formal proof to the appendix. The crux is that
independent of the assignment $h: S \to \{0,1\}$, $\E[Y] \geq
\meanest$ and $\Var(Y) \leq \varest$.  The first part is then a simple
application of the Chebyshev inequality. For the second part, we use
the assumption that $\varest$ is large, to deduce that there exists a
constraint $C$ such that the total weight of constraints that share a
variable from $V \setminus S$ with $C,$ \emph{i.e.}, $\sum_{C_2 \sim_S
  C} \calW(C_2),$ is large. It then follows that at least one variable
$v \in C$ must have large activedegree given $S.$ 
%\Ssnote{Please read
%  this part.}
% \Anote{Not sure
%   how to write this briefly}\Sknote{one/two lines here, + proof should
%   be moved.}

% \Sknote{ Note that I removed this $\alpha$ constant, and the 
% hypothesis that $\E[Y] \geq \meanest$ was removed. In the MAXSAT
% version this condition should be modified, because there it is not obvious that
% $\E[Y]$}

\subsection{Algorithm for Simultaneous \maxcut }

% \Sknote{ we should call this problem MAXCUT, not weighted MAXCUT.. and then the other SDP thing we should call unweighted MAXCUT.}

In Figure~\ref{fig:weighted-maxcut}, we give the algorithm for Simultaneous \maxcut.
The input to the algorithm consists of an integer $k \ge 1,$ $\eps >
0,$ $k$ instances of \maxcut, specified by weight functions
$\calW_1,\ldots,\calW_k,$ and $k$ target objective values
$c_1,\ldots,c_k.$

\begin{figure*}
\begin{tabularx}{\textwidth}{|X|}
\hline
\vspace{0mm}
{\bf Input}: $k$ instances of \maxcut $\calW_1,\ldots,\calW_k$ on the
set of variables $V,$  target objective values $c_1,\ldots,c_k,$ and
$\eps \in (0,\nicefrac{2}{5}].$ \\
{\bf Output}: An assignment to $V.$ \\
{\bf Parameters:}  $\delta_0 = \frac{1}{10k}$, $\epsilon_0 = \frac{\eps}{2}$, $\gamma=\frac{\eps_0^2\delta_0}{16}$, $t = \frac{2k}{\gamma}\cdot\log\left( \frac{11}{\gamma}\right), \alpha = \frac{1}{2}$.
\begin{enumerate}[itemsep=0mm, label=\arabic*.]
\item Initialize $S \leftarrow \emptyset$.
\item For each instance $\ell \in [k]$, initialize $\cnt_\ell
  \leftarrow 0$ and $\flag_\ell \leftarrow \true.$
\item Repeat the following until for every $\ell \in [k]$, either $\flag_\ell = \false$ or
$\cnt_\ell  = t$:
\label{item:alg:max-cut:loop}
\begin{enumerate}
\item For each $\ell \in [k]$, compute
$\varest_\ell = \sum_{C_1 \sim_{S} C_2} \calW_\ell(C_1) \calW_\ell(C_2).$
\item For each $\ell \in [k]$ compute
$\textstyle \meanest_\ell \defeq \frac{1}{2} \sum_{C \in \Act(S)} \calW_\ell(C).$
\item For each $\ell \in [k],$ if $\varest_\ell \geq \delta_0
  \epsilon_0^2 \cdot \meanest_\ell^2 $, then set $\flag_\ell = \true$,
  else set $\flag_\ell = \false$.
\item Choose any $\ell \in [k]$, such that
$\cnt_\ell < t$ AND $\flag_\ell = \true$ (if any):
\label{item:alg:max-cut:high-var}
\begin{enumerate}
\item 
\label{item:alg:max-cut:high-deg}
Find $v \in V$ such that $\activedeg_S(v, \calW_\ell) \geq \gamma
\cdot \activedeg_S(\calW_\ell).$
%\Sknote{I removed the fail .. it is too distracting .. we should remove it everywhere.}
%If no such $v$ exists, output \fail.
\item Set $S \leftarrow S \cup \{v\}.$ We say that $v$ was brought
  into $S$ because of instance $\ell$.
\item Set $\cnt_\ell \leftarrow \cnt_\ell + 1$.
\end{enumerate}
\end{enumerate}
\item 
\label{item:alg:max-cut:random}
Define $g: V \setminus S \to \{0,1\}$ by independently sampling
$g(v) \in \{0,1\}$ with $\E[g(v)] = \nicefrac{1}{2},$ for each $v \in V\setminus S.$
\item 
\label{item:alg:max-cut:partial}
For each partial assignment $h: S \to \{0,1\},$ compute $\out_{h} = \min_{\ell \in [k]}\frac{ \val(h\cup g,
    W_\ell)}{c_\ell}$. If $c_\ell = 0$ for some $\ell \in [k],$ we
  interpret $\frac{\val(h\cup g,\calW_l)}{c_\ell}$ as $+\infty.$
\item Output the largest $\out_{h}$ seen, and the assignment $h\cup g$ that
produced it.
\end{enumerate}
\\ 
\hline
\end{tabularx}
\caption{Algorithm {\algowmaxcut} for approximating weighted simultaneous
  \maxcut}
  \label{fig:weighted-maxcut}
\end{figure*}



\subsection{Analysis of Algorithm \algowmaxcut}
\label{sec:max-cut:analysis}
%\Sknote{Removed the lemma .. made it just text.}
%
First, note that by Lemma~\ref{lemma:max-cut:uvar_lmean_relation},
Step~\ref{item:alg:max-cut:high-deg} in the algorithm always succeeds
in finding a variable $v$.  Next, we note that
Step~\ref{item:alg:max-cut:loop} always terminates. Indeed, whenever
we find an instance $\ell \in [k]$ in
Step~\ref{item:alg:max-cut:high-var} such that $\cnt_\ell < t$ and
$\flag_\ell = \true,$ we increment $\cnt_\ell.$ This can happen only
$tk$ times before the condition $\cnt_\ell < t$ fails for all $\ell
\in [k].$ Thus the loop must terminate within $tk$ iterations.


Let $S^\star$ denote the final set $S$ that we get at the end of
Step~\ref{item:alg:max-cut:loop} of {\algowmaxcut}. To analyze the
approximation guarantee of the algorithm, we classify instances
according to how many vertices were brought into $S^\star$ because of
them.
%
\begin{definition}[Low and high variance instances]
At the completion of Step~\ref{item:alg:max-sat:high-var} in Algorithm
{\algowmaxcut}, if $\ell \in [k]$ satisfies $\cnt_\ell = t$, we call
instance $\ell$ a {\em high variance} instance.  Otherwise we call
instance $\ell$ a \emph{low variance} instance.
\end{definition}
%

% \Sknote{Let us do the perturbation to $h^\star \cup g$, as we do later
%   in the more advanced algorithms.}

% \Sknote{Maybe we should define $S^\star$ to be the set $S$ at the end
%   of the algorithm ? This might make notation much much better,
%   because we keep talking about earlier $S$'s from the middle of the
%   algorithm}

At a high level, the analysis will go as follows: First we analyze
what happens when we give the optimal assignment to $S^\star$ in
Step~\ref{item:alg:max-cut:partial}. For low variance instances, the
cut value of a random assignment to $V \setminus S^\star$ will
concentrate strongly around its expectation, and will give the desired
approximation. For every high variance instance, we will see that many
of its ``heavy-weight" vertices were brought into $S^\star$, and we
will use this to argue that we can cut a large fraction of edges from
these high variance instances by suitably perturbing the optimal
assignment to $S^\star$ to these ``heavy-weight'' vertices. The point
is that one can carry out this perturbation without affecting the
success of the low variance instances.


Let $f^\star: V \to \{0,1\}$ be an assignment such that $\val(f^\star,
\calW_\ell) \geq c_\ell$ for each $\ell$. Let $h^\star = f^\star
|_{S^\star}$. We first show that for low variance instances, when $g :
V \setminus S^\star \to \{0,1\}$ is picked uniformly at random, then
$\val(h^\star \cup g, \calW_\ell)$ is at least $\left(\nfrac{1}{2} -
  \nfrac{\epsilon}{2}\right) \cdot c_\ell$ with high probability.
% \Sknote{Need to write this lemma .. basically take the low variance
% analysis from the proof of the theorem.}
\begin{lemma}
\label{lemma:maxcut:lowvariance}
Let $\ell \in [k]$ be any low variance instance, let $g : V \setminus S^\star \to \{0,1\}$ is picked uniformly at random
Step~\ref{item:alg:max-cut:random} of {\algowmaxcut}. Then the assignment $h^\star
\cup g$ satisfies:
$$ \Pr_{g} \left[ \val(h^\star
\cup g,\calW_\ell) \geq
  (\nicefrac{1}{2}-\nicefrac{\epsilon}{2})\cdot c_\ell \right] \geq 1-\delta_0.$$
\end{lemma}
\begin{proof}
  Since $\ell$ is a {\em low variance} instance, $\flag_{\ell} =
  \false$ when the algorithm terminates. Thus $\varest_\ell <
  \delta_0\epsilon_0^2 \cdot \meanest_\ell^2$.  Let $g: V \to \{0,1\}$
  be the random assignment picked in
  Step~\ref{item:alg:max-cut:random} Define the random
  variable \[Y_\ell \defeq \val(h^\star \cup g,\calW_\ell) -
  \val(h^\star,\calW_\ell).\]

By Lemma~\ref{lemma:max-cut:uvar_lmean_relation}, we know that with probability
  at least $1-\delta_0,$ we have $ Y_\ell \ge (1- \epsilon_0) \E[Y_\ell].$
  Thus, with probability at least $1-\delta_0,$ we have,
\begin{align*}
  \val(h^\star\cup g,\calW_\ell) & = \val(h^\star,\calW_\ell) + Y_\ell \ge
  \val(h^\star,\calW_\ell)  + (1- \epsilon_0) \E[Y_\ell]\\
  & \ge (1-\epsilon_0) \cdot \av[\val(h^\star,\calW_\ell) + Y_\ell] =
  (1-\epsilon_0)\cdot \av[\val(h^\star\cup g,W_\ell)] \\
& \ge \nfrac{1}{2}\cdot (1-\epsilon_0) \cdot \val(f^\star, W_\ell) \\
  & \ge \nfrac{1}{2}\cdot (1-\epsilon_0)\cdot c_\ell \ge
  \left(\nfrac{1}{2} - \nfrac{\eps}{2}\right) \cdot c_\ell ,
\end{align*}
where we have used $\av[\val(h^\star\cup g,W_\ell)] \geq
\nfrac{1}{2}\cdot\val(f^\star, W_\ell),$ since each variable in $g$ is
assigned $\{0,1\}$ independently with probability $\nfrac{1}{2}.$
%\Anote{Used $\eps_0 = \eps$}
\end{proof}

Now we analyze the high variance instances. We prove the following
lemma that proves that at the end of the algorithm, the activedegree
of high variance instances is small, and is dominated by the
activedegree of any variable that was included in $S$ ``early on".
\begin{lemma}
\label{lemma:earlyvariables}
%Let $\gamma= \frac{\epsilon_0^2\delta_0}{16}.$
For all high variance instances $\ell\in [k],$ we have 
\begin{enumerate}
\item $\activedeg_{S^\star}(\calW_\ell) \leq 2(1-\gamma)^t.$ 
\item For each of the first $\nicefrac{t}{2}$ variables that were brought
  inside $S^\star$ because of instance $\ell,$ the total weight of constraints
  incident on each of that variable and totally contained inside $S^\star$ is at
  least $10\cdot\activedeg_{S^\star}(\calW_\ell).$
\end{enumerate}
\end{lemma}
The proof of the lemma is quite simple and is deferred to the
appendix. The crucial observation is that when a variable $u$ is brought
into $S$ because of an instance $\ell,$ the activedegree of $u$ is at
least a $\gamma$ fraction of the total activedegree of instance $\ell.$ Thus,
the activedegree of instance $\ell$ goes down by a multiplicative factor of
$(1-\gamma).$ This immediately implies the first part of the
lemma. For the second part, we use the fact that $t$ is large, and hence the
activedegree of early vertices must be much larger than the final
activedegree of instance $\ell$.
%\Ssnote{@Swastik: Please read this part.}

% By lemma~\ref{lemma:uvar_lmean_relation}, we know that
%   $\activedeg_{S_{u_1}}(u_1,\calW_\ell) \geq \gamma
%   \cdot\activedeg_{S_{u_1}}(\calW_\ell)$. Hence, when we bring that
%   variable into set $S$ the active degree of instance $\ell$ reduces
%   to $(1-\gamma)$ fraction of its current active degree which is at
%   most $2(1-\gamma)$. Continuing this way, we have
%   $\activedeg_{S_{u_i}}(\calW_\ell) \leq 2(1-\gamma)^{i-1}$ for all
%   $i\in [t]$. And hence $\activedeg_S(\calW_\ell) \leq (1-\gamma)^t
%   \cdot \activedeg_{\emptyset}(\calW_\ell) \le 2 (1-\gamma)^t$.

% \Ssnote{Rewrite the part below this.}
% Since $u_t$ is the last vertex that we brought inside $S$, we have $\wt(u_t) \geq \gamma\cdot\activedeg_S(\calW_\ell)$. In general, we have $\wt_{\calW_\ell}(u_i) \geq \gamma(1+\gamma)^{t-i}\cdot\activedeg_S(\calW_\ell)$. And hence, for all $i\in [t/2]$, we have $ \wt_{\calW_\ell}(u_i) \geq \gamma(1+\gamma)^{t/2}\cdot\activedeg_S(\calW_\ell)  = \frac{\gamma}{\sqrt{\delta}}\cdot\activedeg_S(\calW_\ell)$ which is at least $7\cdot\activedeg_S(\calW_\ell)$. Therefore, total weight of $u_i$ inside $S$ is at least $7\cdot\activedeg_S(\calW_\ell) - \activedeg_S(\calW_\ell)$ which is at least $6\cdot\activedeg_S(\calW_\ell)$ as required.


% \Anote{We need to define weight associated with a variable in an instance, using $\wt_{\calW_\ell}$ here}

% \Anote{Will set the expression $2(1-\gamma)^t$ later, update : I don't think we need this}


%\Sknote{ Making changes here for the new perturb algorithm. Please check}
We now describe a procedure {\sc Perturb} (see
Figure~\ref{fig:maxcut-perturb}) which takes $h^\star: S^\star \to \B$ and
$g : V \setminus S^\star \to \B$, and produces 
a new $h : S^\star \to \B$ such that
for all (low variance as well as  high variance) instances $\ell \in [k]$,
$\val(h \cup g, \calW_\ell)$ is not much smaller than $\val(h^\star \cup g, \calW_\ell)$, and 
%$$\val(h \cup g, \calW_\ell) \ge \left(1 - \frac{\epsilon}{2}\right) \cdot \val(h^\star \cup g, \calW_\ell),$$
furthermore, for all high variance instances $\ell \in [k]$, $\val(h
\cup g, \calW_\ell)$ is large. The procedure works by picking a
special variable in $S^\star$ for every { high variance} instance and
perturbing the assignment of $h^\star$ to these special variables. The
partial assignment $h$ is what we will be using to argue that
Step~\ref{item:alg:max-cut:partial} of the algorithm produces a good
Pareto approximation.  More formally, we have the following Lemma.
% \Anote{Are we repeating above things, look at
%   Lemma~\ref{lemma:maxcut_perturbationeffect} } \Sknote{ removed the
%   repetition.}
 %\Sknote { Perturb algorithm + proof of lemma should be changed. should match notation from above.}

\begin{figure*}
\begin{tabularx}{\textwidth}{|X|}
\hline
\vspace{0mm}
{\bf Input}: $h^\star: S^\star \to \B$ and
$g : V \setminus S^\star \to \B$\\
{\bf Output}: A perturbed assignment $h :  S^\star \to \{0,1\}.$ 
%
\begin{enumerate}[itemsep=0mm, label=\arabic*.]
\item Initialize $h \leftarrow h^\star.$
\item For $\ell = 1, \ldots, k$, if instance $\ell$ is a high variance
  instance case (i.e., $\cnt_\ell = t$), we pick a special variable
  $v_\ell \in S^\star$ associated to this instance as follows:
\begin{enumerate}
\item Let $B = \{ v \in V \mid \exists \ell \in [k] \mbox{ with }
  \sum_{C \in \calC, C \owns v} \calW_{\ell}(C)\cdot C(h \cup g) \geq
  \frac{\epsilon}{2k} \cdot\val(h\cup g, \calW_\ell) \}$.  Since the weight of
  each constraint is counted at most twice, we know that $|B| \leq \frac{4k^2}{\epsilon}$.
\item Let $U$ be the set consisting of the first $t/2$ variables
brought into $S^\star$ because  of instance $\ell$.
\item Since $\nfrac{t}{2} > |B|+ k$, there exists some $u \in U$
  such that $u \not\in B \cup \{v_1, \ldots, v_{\ell-1}\}$.  We define
  $v_\ell$ to be $u$.
\item By Lemma~\ref{lemma:earlyvariables}, the total $\calW_\ell$ weight of constraints that are incident on $v_\ell$
  and only containing variables from $S^\star$ is at least
 % $\wt_{\calW_\ell}(v_\ell) \geq
  $10\cdot\activedeg_{S^\star}(\calW_\ell)$. We update $h$ by 
setting $h(v_\ell)$ to be that value from $\{0,1\}$
such that at least half of the $\calW_\ell$ weight of these constraints is
  satisfied.
\end{enumerate}
\item Return the assignment $h.$
%%\vspace{-3mm}
\end{enumerate}
% \Anote{ Shall we call the final $f|_S$ with some different name, as we
%   are not using the notation $f|_S$ in the later sections. Also, $f$
%   seems more general name for this special assignment}
\\
\hline
\end{tabularx}
\caption{Procedure {\sc Perturb} for perturbing the optimal
  assignment}
  \label{fig:maxcut-perturb}
\end{figure*}

\begin{lemma}
\label{lemma:maxcut_perturbationeffect} 
For the assignment $h$ obtained from Procedure {\sc Perturb} (see
Figure~\ref{fig:maxcut-perturb}), for each $\ell\in [k]$, $\val(h\cup
g,\calW_\ell) \geq (1-\nicefrac{\epsilon}{2}) \cdot \val(h^\star \cup
g, \calW_\ell)$. Furthermore, for each {\em high variance} instance
$\calW_\ell$, $\val(h\cup g,\calW_\ell) \geq
4 \cdot \activedeg_{S^\star}(\calW_\ell).$
\end{lemma}
\begin{proof}
  Consider the special variable $v_\ell$ that we choose for {\em high
    variance} instance $\ell \in [k]$. Since $v_\ell \notin B,$ the
  constraints incident on $v_\ell$ only contribute at most a
  $\nfrac{\eps}{2k}$ fraction of the objective value in each
  instance. 
  % all variables $v$ such that if we change the value of $v$ given by
  % $h\cup g$ then it reduces the objective value of some instance by at
  % least $\frac{\epsilon}{2k}$ fraction of it's current value. Since
  % $v_\ell$ is not present in $B$, 
  Thus, changing the assignment $v_\ell$ can reduce the value of any
  instance by at most a $\frac{\epsilon}{2k}$ fraction of their
  current objective value. Also, we pick different special variables
  for each {\em high variance} instance. Hence, the total effect of
  these perturbations on any instance is that it reduces the objective
  value (given by $h^\star \cup g$) by at most $1 - (1-
  \frac{\epsilon}{2k})^k \le \frac{\epsilon}{2}$ fraction.  Hence for
  all instances $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq
  (1-\nicefrac{\epsilon}{2})\cdot\val(h^\star\cup g,\calW_\ell)$.

  For a {\em high variance instance} $\ell \in [k]$, since $v_\ell \in
  U,$ the variable $v_\ell$ must be one of the first $\nfrac{t}{2}$
  variables brought into $S^\star$ because of $\ell.$ Hence, by
  Lemma~\ref{lemma:earlyvariables} the total weight of constraints
  that are incident on $v_\ell$ and entirely contained inside
  $S^\star$ is at least
  $10\cdot\activedeg_{S^\star}(\calW_\ell)$. Hence, there is an
  assignment to $v_\ell$ that satisfies at least at least half the
  weight of these \maxcut constraints\footnote{This is true even if
    the constraints were \maxsat constraint, but not if they are
    \maxand constraints.} in $\ell.$ At the end of the iteration when
  we pick an assignment to $v_\ell,$ we have $\val(h\cup g,
  \calW_\ell) \ge 5\cdot\activedeg_{S^\star}(\calW_\ell).$ Since the
  later perturbations do not affect value of this instance by more
  than $\nfrac{\epsilon}{2}$ fraction, we get that for the final
  assignment $h$, $\val(h\cup g,\calW_\ell) \ge
  (1-\nfrac{\epsilon}{2})\cdot 5 \cdot
  \activedeg_{S^\star}(\calW_\ell) \geq 4\cdot
  \activedeg_{S^\star}(\calW_\ell).$
%  Since the total weight of constraints incident on $V \setminus S$ is
%  bounded by $\activedeg_{S^\star}(\calW_\ell),$ we get $\val(h, \calW_\ell)
%  \ge 3\cdot \activedeg_{S^\star}(\calW_\ell).$
\end{proof}

Given these lemmas, we will now show that our algorithm finds an
assignment that gives an objective value at least
$(\nfrac{1}{2}-\epsilon) c_\ell$ weight in each instance $\ell \in
[k],$ with high probability.
%
%\Sknote{the proof of this probably gets shorter now.}
\begin{theorem}
\label{thm:max-cut}
Suppose we're given $\eps \in (0,\nfrac{2}{5}],$ $k$ simultaneous
\maxcut instances $\calW_1, \ldots, \calW_\ell$ on $n$ variables, and
target objective value $c_1, \ldots,c_k$ with the guarantee that there
exists an assignment $f^\star$ such that for each $\ell \in [k],$ we
have $\val( f^\star, \calW_\ell) \ge c_\ell.$ Then, the algorithm {\algowmaxcut} runs in time $\exp(\nfrac{k^3}{\eps^2}\log
(\nfrac{k}{\eps^2}))\cdot\poly(n),$ and with probability at least
$0.9,$ outputs an assignment $f$ such that for each $\ell \in [k],$ we
have, $\val(f, \calW_\ell) \ge \left( \frac{1}{2} -\epsilon\right)
\cdot c_\ell.$
\end{theorem}
\begin{proof}
  % \Anote{Please go through this analysis to check if it is following
  %   clearly, I made it similar to the one in maxcsp section} Recall
  % that $h^\star = f^\star|_{S^\star}.$ 
  By Lemma~\ref{lemma:maxcut:lowvariance} and a union bound, with
  probability at least $1 -k\delta_0 > 0.9$, over the choice of $g$,
  we have that for {\em every} low variance instance $\ell \in [k]$,
  $\val(h^\star \cup g, \calW_\ell) \geq (\nfrac{1}{2} -
  \nfrac{\epsilon}{2}) \cdot c_{\ell}$. Henceforth we assume that the
  assignment $g$ sampled in Step~\ref{item:alg:max-cut:random} of the
  algorithm is such that this event occurs. Let $h$ be the output of
  the procedure {\sc Perturb} given in Figure~\ref{fig:maxcut-perturb}
  for the input $h^\star$ and $g.$
% \Anote{Should we name for this special g and h?}.
  By Lemma~\ref{lemma:maxcut_perturbationeffect}, $h$ satisfies
\begin{enumerate}
\item\label{item:maxcut:proof:guarantees:1} For every instance $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq (1-\nfrac{\eps}{2})\cdot \val(h^\star\cup g,\calW_\ell).$
\item \label{item:maxcut:proof:guarantees:2}For every high variance
  instance $\ell \in [k]$, $\val(h\cup g,\calW_\ell) \geq
 4 \cdot  \activedeg_{S^\star}(\calW_\ell).$
\end{enumerate}
%Since we are trying all assignment to $S^\star$, we will be 
We now show that the desired Pareto approximation behavior is achieved
when $h$ is considered as the partial assignment in
Step~\ref{item:alg:max-cut:partial} of the algorithm. We analyze the
guarantee for low and high variance instances separately.
% when we consider this perturbed assignment in Step~\ref{item:alg:max-cut:partial}. 

For any {\em low variance} instance $\ell \in [k],$ from
property~\ref{item:maxcut:proof:guarantees:1} above, we have
$\val(h\cup g,\calW_\ell) \geq (1-\nfrac{\eps}{2})\cdot
\val(h^\star\cup g,\calW_\ell)$. Since we know that $\val(h^\star \cup
g, \calW_\ell) \geq (\nfrac{1}{2}-\nfrac{\eps}{2})\cdot c_\ell$, we
have $\val(h\cup g,\calW_\ell) \geq (\nfrac{1}{2}-\eps)\cdot c_\ell$.

For every high variance instance $\ell \in [k],$ since $h^\star =
f^\star|_{S^\star},$ for any $g$ we must have,
\[\val(h^\star \cup g, \calW_\ell) \ge \val(f^\star, \calW_\ell) -
\activedeg_{S^\star}(\calW_\ell) \ge c_\ell - \activedeg_{S^\star}(\calW_\ell) .\]
Combining this with properties~\ref{item:maxcut:proof:guarantees:1}
and \ref{item:maxcut:proof:guarantees:2} above, we get,
\begin{align*}
\val(h \cup g, \calW_\ell) &\ge \left( 1 - \nfrac{\epsilon}{2}
\right) \cdot \max\{c_\ell - \activedeg_{S^\star}(\calW_\ell), 4 \cdot
\activedeg_{S^\star}(\calW_\ell)\} \\
&\ge \left( \nfrac{1}{2} - \epsilon \right) \cdot c_\ell.
\end{align*}

Thus, for all instances $\ell \in [k]$, we get $\val(h \cup g) \ge
\left(\nfrac{1}{2}-\eps\right) \cdot c_{\ell}.$ Since we are taking
the best assignment $h\cup g$ at the end of the algorithm {\algowmaxcut}, the theorem follows.
%By Lemma~\ref{lemma:max-cut:uvar_lmean_relation}, we know that with probability
%  at least $1-\delta_0,$ we have $ Y_\ell \ge (1- \epsilon_0) \E[Y_\ell].$
%  Thus, with probability at least $1-\delta_0,$ we have,
%\begin{align*}
%  \val(f|_S\cup g,\calW_\ell) & = \val(f|_S,\calW_\ell) + Y_\ell \ge
%  \val(f|_S,\calW_\ell)  + (1- \epsilon_0) \E[Y_\ell]\\
%  & \ge (1-\epsilon_0) \cdot \av[\val(f|_S,\calW_\ell) + Y_\ell] =
%  (1-\epsilon_0)\cdot \av[\val(f|_S\cup g,W_\ell)] \\
%& \ge \nfrac{1}{2}\cdot (1-\epsilon_0) \cdot \val(f, W_\ell) \\
%  & \ge \nfrac{1}{2}\cdot (1-\epsilon_0) (1-\nicefrac{\eps}{2}) \cdot c_\ell \ge
%  \left(\nfrac{1}{2} - \epsilon_0 - \nicefrac{\eps}{2}\right) \cdot c_\ell = \left(\nfrac{1}{2} - \eps\right) \cdot c_\ell ,
%\end{align*}
%where we have used $\av[\val(f|_S\cup g,W_\ell)] \geq
%\nfrac{1}{2}\cdot\val(f, W_\ell),$ since each variable in $g$ is
%assigned $\{0,1\}$ independently with probability $\nfrac{1}{2}.$
% % $\E[Y] \geq \frac{3}{4} Y_h$ ~\cite{GW-maxsat}
% %  \Anote{shall we write the proof of this may be in Appendix? or this
% %    is okay}, where $Y_h$ is an upper bound of the optimal value of
% %  $Y$ that we get after extending assignment $f^\star|_{S}$ to $V\setminus
% %  S$ i.e $Y_h \geq \opt$ \Anote{check if I am doing any mistakes
% %    here}. By lemma~\ref{lemma:uvar_lmean_relation}, we thus have
% %  $\Pr[ Y < (1- \epsilon_0) \E[Y] ] < \delta_0$. And since, changing
% %  assignment $f^\star_{|S}$ to $f|_{S}$, as given by {\em Procedure} $1$,
% %  reduces the value of any instance $\ell\in [k]$ by at most
% %  $\epsilon\cdot \val(f^\star,\calW_\ell)$, we get a
% %  $\left(\frac{3}{4}-\epsilon - \frac{3\epsilon_0}{4}\right)$
% %  approximate solution with probability at least $(1-\delta_0)$.
%Hence, by a union bound, we get an objective value of at least
%$\left(\frac{1}{2} -\epsilon\right)\cdot c_\ell,$ for every {\em low
%  variance instance} with probability at least $1-k\delta_0 = 0.9$.

{\bf Running time : } 
Running time of the algorithm is $2^{O(kt)}\cdot\poly(n)$ which is $\exp(\nfrac{k^3}{\eps^2}\log (\nfrac{k}{\eps^2}))\cdot\poly(n)$.
\Ssnote{Can we do a more careful analysis of the running time?}
\end{proof}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "new-simopt"
%%% End: 

